SPIRou Input Catalogue: Global properties of 440 M dwarfs observed with ESPaDOnS at CFHT

Present and future high-precision radial-velocity spectrometers dedicated to the discovery of low-mass planets orbiting low-mass dwarfs need to focus on the best selected stars to make an efficient use of telescope time. In the framework of the preparation of the SPIRou Input Catalog, the CoolSnap program aims at screening M dwarfs in the solar neighborhood against binarity, rapid rotation, activity, ... To optimize the selection, the present paper describes the methods used to compute effective temperature, metallicity, projected rotation velocity of a large sample of 440 M dwarfs observed in the visible with the high-resolution spectro-polarimeter ESPaDOnS at CFHT. It also summarizes known and newly-discovered spectroscopic binaries, and stars known to belong to visual multiple systems. A calibration of the projected rotation velocity versus measured line widths for M dwarfs observed by the ESPaDOnS spectro-polarimeter is derived, and the resulting values are compared to equatorial rotation velocities deduced from rotation periods and radii. A comparison of the derived effective temperatures and metallicities with literature values is also conducted. Finally, the radial velocity uncertainty of each star in the sample is estimated, to narrow down the selection of stars to be included into the SPIRou Input Catalogue (SPIC).

==> vsini.tex <==
2MASS    & JD     &  SNR &  Teff & [Fe/H] & $\sigma_{LSD}$ & $\sigma_{FeH}$ \\
         &-2400000& 809nm&  K    &       &  km/s          & km/s   \\
\hline
   J00182549+4401376 &  57610.13 &   191 &      3347 &     -0.43 &    4.58 &     1.998 \\
   J00182549+4401376 &  57611.14 &   195 &      3345 &     -0.37 &    4.56 &     2.030 \\
   J00182549+4401376 &  57677.80 &   338 &      3330 &     -0.39 &    4.50 &     2.502 \\
   J00294322+0112384 &  56967.84 &   189 &      3609 &     -0.12 &    4.14 &     2.591 \\
   J00294322+0112384 &  56906.02 &   168 &      3684 &     -0.13 &    4.12 &     1.699 \\
   J00385879+3036583 &  57263.99 &   286 &      3468 &     -0.09 &    4.02 &     1.941 \\
   J00385879+3036583 &  57326.87 &   320 &      3476 &     -0.07 &    3.99 &     2.372 \\
   J00570261+4505099 &  57344.70 &   317 &      3337 &     -0.04 &    4.07 &     2.090 \\
   J00570261+4505099 &  57358.72 &   318 &      3374 &     -0.05 &    4.03 &     2.184 \\
   J00582789-2751251 &  57262.02 &   255 &      3316 &     -0.00 &    3.84 &     2.250 \\
   J00582789-2751251 &  57284.93 &   216 &      3335 &      0.05 &    3.87 &     2.198 \\
   J01012006+6121560 &  56907.05 &   324 &      3474 &     -0.22 &    4.15 &     2.228 \\
   J01012006+6121560 &  56917.01 &   299 &      3501 &     -0.20 &    4.15 &     2.332 \\
   J01023213+7140475 &  56883.96 &   325 &      3439 &      0.07 &    3.93 &     1.898 \\
   J01023213+7140475 &  56904.12 &   368 &      3461 &      0.05 &    3.89 &     1.729 \\
   J01123052-1659570 &  57652.84 &   200 &    -32768 &         - &    5.45 &     2.880 \\
   J01123052-1659570 &  57673.96 &   203 &      3303 &     -0.28 &    5.69 &     2.349 \\
   J01432015+0419172 &  56908.12 &   320 &      3488 &     -0.08 &    4.06 &     2.336 \\
   J01432015+0419172 &  56968.88 &   222 &      3398 &     -0.05 &    4.10 &     2.004 \\
   J01432015+0419172 &  56968.89 &   223 &      3411 &     -0.10 &    4.11 &     1.966 \\
   J01432015+0419172 &  56968.92 &   251 &      3429 &     -0.09 &    4.08 &     1.770 \\
   J01515108+6426060 &  57330.81 &   283 &      3533 &      0.12 &    4.05 &     2.278 \\
   J01515108+6426060 &  57348.73 &   187 &      3616 &      0.11 &    4.01 &     2.093 \\
   J02013533+6346118 &  56907.07 &   323 &      3417 &      0.16 &    3.86 &     2.117 \\
   J02013533+6346118 &  56917.02 &   319 &      3432 &      0.16 &    3.84 &     2.481 \\
   J02441245-1321387 &  56909.09 &    77 &      2850 &     -0.07 &    7.44 &         - \\
   J02441245-1321387 &  56909.10 &    96 &      2798 &      0.00 &    7.12 &         - \\
   J02441245-1321387 &  56909.12 &   110 &      2792 &     -0.05 &    6.94 &     1.942 \\
   J02441245-1321387 &  56967.86 &   135 &      2861 &      0.00 &    7.23 &     1.925 \\
   J02441537+2531249 &  56883.98 &   263 &      3383 &     -0.08 &    4.00 &     1.861 \\
   J02441537+2531249 &  56904.12 &   327 &      3389 &     -0.08 &    3.98 &     2.163 \\
   J03143273+5926160 &  57348.76 &   250 &      3444 &      0.07 &    4.01 &     2.282 \\
   J03143273+5926160 &  57403.82 &   263 &      3444 &      0.08 &    4.06 &     2.028 \\
   J03531041+6234081 &  57262.05 &   331 &      3461 &     -0.23 &    4.09 &     2.063 \\
   J03531041+6234081 &  57285.03 &   280 &      3449 &     -0.23 &    4.05 &     1.981 \\
   J04311147+5858375 &  57437.78 &   306 &      3086 &      0.14 &    3.73 &     2.039 \\
   J04311147+5858375 &  57475.76 &   223 &      3202 &      0.08 &    3.85 &     1.999 \\
   J04425586+2128230 &  57262.07 &   329 &      3359 &      0.11 &    3.94 &     2.051 \\
   J04425586+2128230 &  57285.07 &   295 &      3331 &      0.06 &    3.92 &     1.990 \\
   J05031607+2123563 &  57264.02 &   270 &       957 &      0.00 &   15.81 &         - \\
   J05031607+2123563 &  57326.93 &   302 &      2199 &     -0.13 &    4.29 &     2.490 \\
   J05032009-1722245 &  57262.10 &   288 &      3364 &     -0.18 &    4.12 &     2.082 \\
   J05032009-1722245 &  57289.14 &   231 &      3325 &     -0.16 &    4.13 &     1.968 \\
   J05124223+1939566 &  56968.98 &   380 &      3535 &     -0.09 &    3.99 &     2.249 \\
   J05124223+1939566 &  57109.72 &   403 &      3548 &     -0.10 &    4.03 &     2.046 \\
   J05280015+0938382 &  57330.95 &   271 &      3306 &     -0.24 &    4.26 &     2.259 \\
   J05280015+0938382 &  57330.98 &   301 &      3283 &     -0.17 &    4.25 &     2.263 \\
   J05280015+0938382 &  57438.81 &   203 &      3242 &     -0.19 &    4.18 &     2.215 \\
   J05345212+1352471 &  57264.12 &   220 &      3298 &      0.01 &    3.92 &     2.104 \\
   J05345212+1352471 &  57326.95 &   306 &      3267 &      0.01 &    3.86 &     2.123 \\
   J05420897+1229252 &  56972.91 &   486 &      3175 &     -0.16 &    4.07 &     2.141 \\
   J05420897+1229252 &  57402.99 &   310 &      3186 &     -0.14 &    4.20 &     1.842 \\
   J05420897+1229252 &  57401.91 &   313 &      3202 &     -0.17 &    4.17 &     2.206 \\
   J05420897+1229252 &  57328.93 &   535 &      3183 &     -0.14 &    4.01 &     2.113 \\
   J06011106+5935508 &  57107.73 &   513 &      3218 &     -0.05 &    3.99 &     2.191 \\
   J06011106+5935508 &  57035.05 &   507 &      3199 &     -0.02 &    3.93 &     2.107 \\
   J06101978+8206256 &  57108.72 &   304 &      3432 &     -0.08 &    4.04 &     2.170 \\
   J06101978+8206256 &  57328.00 &   341 &      3491 &     -0.09 &    3.99 &     1.898 \\
   J07100298-0133146 &  56970.95 &   143 &      3874 &      1.25 &    4.97 &         - \\
   J07100298-0133146 &  57032.11 &   136 &      3877 &      1.27 &    4.93 &         - \\
   J07272450+0513329 &  56973.08 &   520 &      3211 &     -0.05 &    3.93 &     2.081 \\
   J07272450+0513329 &  57014.13 &   499 &      3220 &     -0.04 &    3.96 &     2.001 \\
   J07284541-0317524 &  57264.14 &   191 &      3401 &     -0.03 &    3.91 &     2.113 \\
   J07284541-0317524 &  57328.12 &   293 &      3370 &     -0.01 &    3.85 &     2.078 \\
   J07315735+3613477 &  57439.77 &   489 &      3394 &      0.11 &    4.59 &     2.139 \\
   J07315735+3613477 &  57472.84 &   221 &      3391 &      0.14 &    4.73 &     2.217 \\
   J07315735+3613477 &  57472.85 &   228 &      3411 &      0.15 &    4.68 &     2.208 \\
   J07345632+1445544 &  57014.16 &   294 &    -32768 &         - &    5.78 &     3.009 \\
   J07345632+1445544 &  57035.12 &   304 &    -32768 &         - &    5.74 &     3.523 \\
   J07384089-2113276 &  57436.80 &   204 &      3401 &     -0.23 &    4.06 &     1.800 \\
   J07384089-2113276 &  57413.98 &   266 &      3383 &     -0.17 &    4.10 &     2.044 \\
   J07581269+4118134 &  57011.13 &   473 &      3178 &      0.02 &    3.83 &     2.055 \\
   J07581269+4118134 &  57033.09 &   475 &      3176 &      0.04 &    3.84 &     2.053 \\
   J08160798+0118091 &  57011.16 &   359 &      3527 &     -0.08 &    4.15 &     1.980 \\
   J08160798+0118091 &  57032.12 &   400 &      3552 &     -0.10 &    4.12 &     1.987 \\
   J08405923-2327232 &  57035.09 &   393 &      3268 &      0.21 &    3.94 &     2.260 \\
   J08405923-2327232 &  57032.98 &   337 &      3248 &      0.25 &    3.93 &     2.051 \\
   J09201112-0110171 &  57526.74 &   159 &      2226 &      0.09 &    6.06 &         - \\
   J09304457+0019214 &  57037.06 &   320 &      3306 &     -0.01 &    4.09 &     2.123 \\
   J09304457+0019214 &  57022.07 &   364 &      3276 &     -0.06 &    4.13 &     2.072 \\
   J09360161-2139371 &  57031.14 &   368 &      3433 &     -0.23 &    4.04 &     2.175 \\
   J09360161-2139371 &  57084.91 &   352 &      3439 &     -0.24 &    4.08 &     2.164 \\
   J09423493+7002024 &  56973.13 &   385 &      3493 &      0.16 &    4.24 &     2.196 \\
   J09423493+7002024 &  57012.16 &   348 &      3480 &      0.20 &    4.24 &     2.067 \\
   J09541556+2025328 &  57527.79 &   201 &      3361 &     -0.04 &    4.92 &     2.309 \\
   J09541556+2025328 &  57527.74 &   113 &      3019 &     -0.05 &    5.67 &     2.744 \\
   J10112218+4927153 &  57115.87 &   240 &      4156 &      0.83 &    4.48 &     1.959 \\
   J10112218+4927153 &  57115.87 &   306 &      4146 &      0.85 &    4.49 &     1.892 \\
   J10112218+4927153 &  57107.77 &   547 &      4179 &      0.83 &    4.49 &     2.307 \\
   J10112218+4927153 &  57115.86 &   182 &      4129 &      0.87 &    4.47 &     1.935 \\
   J10123481+5703495 &  57439.82 &   276 &      3269 &     -0.05 &    4.01 &     2.280 \\
   J10123481+5703495 &  57472.89 &   222 &      3317 &     -0.11 &    3.98 &     2.355 \\
   J10164599-1157412 &  57022.12 &   329 &      3473 &      0.14 &    3.89 &     2.170 \\
   J10164599-1157412 &  57014.17 &   303 &      3466 &      0.08 &    3.90 &     2.112 \\
   J10164599-1157412 &  57403.02 &   325 &      3507 &      0.08 &    3.89 &     2.051 \\
   J10285555+0050275 &  57031.16 &   287 &      3501 &     -0.12 &    4.13 &     2.143 \\
   J10285555+0050275 &  57021.10 &   356 &      3498 &     -0.10 &    4.16 &     2.004 \\
   J10285555+0050275 &  57328.16 &   357 &      3465 &     -0.12 &    4.15 &     1.886 \\
   J10550557+0559430 &  57497.82 &   200 &    -32768 &         - &    5.20 &     2.649 \\
   J11000432+2249592 &  57021.11 &   314 &      3446 &     -0.07 &    4.14 &     2.309 \\
   J11000432+2249592 &  57031.16 &   295 &      3452 &     -0.14 &    4.15 &     2.131 \\
   J11000432+2249592 &  57330.16 &   388 &      3432 &     -0.06 &    4.07 &     2.110 \\
   J11032023+3558117 &  56973.16 &   480 &      3538 &     -0.40 &    4.06 &     2.066 \\
   J11032023+3558117 &  56973.16 &   479 &      3527 &     -0.39 &    4.04 &     2.115 \\
   J11032023+3558117 &  57012.14 &   473 &      3523 &     -0.41 &    4.07 &     2.238 \\
   J11110245+3026415 &  57108.75 &   284 &      3724 &      0.27 &    4.06 &     2.382 \\
   J11110245+3026415 &  57121.03 &   205 &      3707 &      0.29 &    4.05 &     2.412 \\
   J11330051-1531543 &  57525.82 &   172 &    -32768 &         - &   13.01 &     7.175 \\
   J11414471+4245072 &  57035.16 &   424 &      3174 &      0.10 &    3.74 &     1.988 \\
   J11414471+4245072 &  57080.89 &   354 &      3175 &      0.11 &    3.78 &     2.029 \\
   J11421096+2642251 &  57032.14 &   323 &      3439 &      0.03 &    3.86 &     2.078 \\
   J11421096+2642251 &  57080.92 &   301 &      3451 &      0.01 &    3.89 &     2.124 \\
   J11473762+0501106 &  57497.89 &   199 &    -32768 &         - &   10.92 &         - \\
   J11474440+0048164 &  57022.10 &   409 &      3172 &     -0.09 &    4.24 &     2.225 \\
   J11474440+0048164 &  57031.18 &   359 &      3155 &     -0.09 &    4.19 &     2.300 \\
   J12100559-1504156 &  57037.12 &   481 &      3122 &      0.23 &    3.76 &     1.872 \\
   J12100559-1504156 &  57407.14 &   433 &      3102 &      0.20 &    3.78 &     1.852 \\
   J12140866-2345172 &  57474.86 &   209 &    -32768 &         - &   18.19 &         - \\
   J12385241+1141461 &  57037.09 &   393 &      3330 &      0.24 &    3.82 &     1.775 \\
   J12385241+1141461 &  57406.05 &   391 &      3313 &      0.22 &    3.88 &     2.070 \\
   J12435889-1614351 &  57475.95 &   146 &    -32768 &         - &    8.07 &     4.198 \\
   J12475664+0945050 &  57080.94 &   396 &      3181 &      0.02 &    3.81 &     2.026 \\
   J12475664+0945050 &  57037.16 &   417 &      3209 &      0.06 &    3.81 &     1.938 \\
   J12490273+6606366 &  57406.12 &   467 &      2329 &     -0.13 &    5.16 &     2.907 \\
   J12490273+6606366 &  57436.12 &   358 &      1858 &     -0.10 &    6.93 &     5.332 \\
   J13282106-0221365 &  57408.13 &   330 &      3401 &      0.14 &    3.86 &     2.141 \\
   J13282106-0221365 &  57236.76 &   282 &      3375 &      0.13 &    3.78 &     2.099 \\
   J13424328+3317255 &  57084.95 &   339 &      3225 &     -0.03 &    4.01 &     2.270 \\
   J13424328+3317255 &  57406.09 &   395 &      3196 &     -0.04 &    4.01 &     2.147 \\
   J13455074-1758047 &  57439.04 &   379 &      3262 &      0.06 &    3.88 &     2.259 \\
   J13455074-1758047 &  57236.74 &   330 &      3243 &      0.07 &    3.79 &     1.953 \\
   J13455096-1209502 &  57441.07 &   195 &      3927 &      0.39 &    4.34 &     1.789 \\
   J13455096-1209502 &  57471.95 &   189 &      3871 &      0.42 &    4.34 &     1.893 \\
   J14172209+4525461 &  57475.88 &   186 &    -32768 &         - &   13.69 &     8.846 \\
   J14341683-1231106 &  57406.17 &   442 &      3075 &      0.15 &    3.70 &     1.934 \\
   J14341683-1231106 &  57417.02 &   379 &      3130 &      0.15 &    3.74 &     1.955 \\
   J15192689-0743200 &  57085.03 &   328 &      3356 &     -0.08 &    4.06 &     2.179 \\
   J15192689-0743200 &  57032.18 &   289 &      3326 &     -0.14 &    3.98 &     1.976 \\
   J16164537+6715224 &  57033.16 &   299 &      3451 &      0.19 &    3.95 &     2.189 \\
   J16164537+6715224 &  57085.16 &   281 &      3398 &      0.14 &    3.95 &     2.159 \\
   J16240913+4821112 &  57226.77 &   362 &      3467 &     -0.42 &    4.07 &     2.507 \\
   J16240913+4821112 &  57402.18 &   348 &      3485 &     -0.41 &    4.08 &     2.386 \\
   J16252459+5418148 &  57033.17 &   311 &      3470 &     -0.40 &    4.34 &     2.182 \\
   J16252459+5418148 &  57205.79 &   324 &      3475 &     -0.38 &    4.26 &     2.493 \\
   J16275072-1926069 &  57559.76 &   193 &      3607 &      1.74 &    3.85 &         - \\
   J16301808-1239434 &  57559.77 &   219 &      3284 &      0.05 &    3.94 &     1.855 \\
   J17093153+4340531 &  57085.13 &   347 &      2798 &      0.22 &    3.79 &     2.053 \\
   J17093153+4340531 &  57121.13 &   358 &      2804 &      0.16 &    3.82 &     2.091 \\
   J17195422+2630030 &  57441.16 &   258 &    -32768 &         - &    4.83 &     2.408 \\
   J17195422+2630030 &  57406.15 &   280 &    -32768 &         - &    4.81 &     2.415 \\
   J17195422+2630030 &  57442.10 &   216 &    -32768 &         - &    4.88 &     2.363 \\
   J17294104-1748323 &  57085.17 &   514 &      4803 &      3.11 &    4.74 &         - \\
   J17294104-1748323 &  57120.15 &   368 &      4466 &      2.65 &    4.46 &         - \\
   J17362594+6820220 &  56884.93 &   423 &      3394 &     -0.03 &    3.86 &     2.050 \\
   J17362594+6820220 &  56903.77 &   492 &      3385 &     -0.02 &    3.86 &     2.023 \\
   J17435595+4322441 &  56886.81 &   205 &      3517 &      0.08 &    3.99 &     2.302 \\
   J17435595+4322441 &  56912.73 &   243 &      3491 &      0.04 &    3.97 &     1.997 \\
   J17462934-0842362 &  57226.78 &   121 &    -32768 &         - &    4.85 &         - \\
   J17462934-0842362 &  57328.68 &   129 &      1817 &     -0.06 &    7.49 &     5.734 \\
   J17574849+0441405 &  57616.81 &   213 &      3360 &     -0.55 &    4.67 &     2.589 \\
   J17574849+0441405 &  57677.77 &   200 &      3460 &     -0.47 &    4.75 &     2.184 \\
   J17575096+4635182 &  57289.82 &   221 &      3369 &      0.06 &    3.97 &     2.136 \\
   J17575096+4635182 &  57328.70 &   284 &      3354 &      0.05 &    3.98 &     2.082 \\
   J18151241-1924063 &  56912.72 &   284 &      3612 &     -0.03 &    4.12 &     2.515 \\
   J18151241-1924063 &  57229.89 &   318 &      3593 &     -0.05 &    4.12 &     2.068 \\
   J18302580-0006226 &  57677.78 &    69 &      2716 &      0.80 &    3.91 &         - \\
   J18302580-0006226 &  57652.75 &   110 &      2652 &      0.76 &    3.86 &         - \\
   J18410977+2447143 &  57351.71 &   365 &      2149 &      0.00 &    4.45 &     2.562 \\
   J18410977+2447143 &  57328.73 &   382 &      2148 &      0.04 &    4.44 &     2.422 \\
   J18415908+3149498 &  57328.75 &   280 &      3400 &     -0.15 &    3.99 &     2.168 \\
   J18415908+3149498 &  57287.82 &   206 &      3445 &     -0.12 &    4.02 &     2.088 \\
   J18415908+3149498 &  57226.95 &   277 &      3423 &     -0.13 &    3.96 &     1.949 \\
   J18415908+3149498 &  57263.83 &   276 &      3427 &     -0.14 &    3.99 &     2.039 \\
   J18424666+5937499 &  57328.71 &   376 &      3392 &     -0.27 &    4.02 &     2.220 \\
   J18424666+5937499 &  57205.80 &   395 &      3441 &     -0.30 &    4.02 &     2.073 \\
   J18450905-0926438 &  57615.83 &   187 &      4340 &      2.51 &    5.26 &         - \\
   J18450905-0926438 &  57652.80 &   191 &      4418 &      2.52 &    5.28 &         - \\
   J19071320+2052372 &  57330.72 &   238 &      3504 &     -0.41 &    4.15 &     2.109 \\
   J19071320+2052372 &  56908.89 &   241 &      3436 &     -0.41 &    4.14 &     2.096 \\
   J19071320+2052372 &  56908.92 &   215 &      3438 &     -0.40 &    4.14 &     2.022 \\
   J19071320+2052372 &  56908.94 &   289 &      3438 &     -0.40 &    4.15 &     2.202 \\
   J19071320+2052372 &  56972.70 &   441 &      3481 &     -0.46 &    4.14 &     2.080 \\
   J19082996+3216520 &  57233.08 &   228 &      3325 &     -0.09 &    3.98 &     2.233 \\
   J19082996+3216520 &  57330.74 &   203 &      3383 &     -0.10 &    4.04 &     2.219 \\
   J19082996+3216520 &  57297.84 &   188 &      3348 &     -0.01 &    4.00 &     2.065 \\
   J20303207+6526586 &  56889.04 &   310 &      3400 &     -0.05 &    4.17 &     2.328 \\
   J20303207+6526586 &  56903.91 &   323 &      3407 &     -0.05 &    4.19 &     2.208 \\
   J20303207+6526586 &  57603.95 &   309 &      3413 &     -0.04 &    4.14 &     2.392 \\
   J20303207+6526586 &  57606.97 &   299 &      3412 &     -0.05 &    4.17 &     2.013 \\
   J20303207+6526586 &  57607.94 &   310 &      3441 &     -0.07 &    4.16 &     2.371 \\
   J20303207+6526586 &  57608.94 &   311 &      3395 &     -0.08 &    4.17 &     2.191 \\
   J20303207+6526586 &  57609.97 &   308 &      3427 &     -0.04 &    4.18 &     2.073 \\
   J20303207+6526586 &  57610.97 &   308 &      3416 &     -0.00 &    4.20 &     2.297 \\
   J20303207+6526586 &  57611.88 &   310 &      3422 &     -0.07 &    4.19 &     2.159 \\
   J20303207+6526586 &  57612.90 &   343 &      3414 &     -0.07 &    4.19 &     2.195 \\
   J20303207+6526586 &  57613.96 &   309 &      3405 &     -0.07 &    4.21 &     2.232 \\
   J20303207+6526586 &  57616.82 &   342 &      3423 &     -0.06 &    4.19 &     2.185 \\
   J20303207+6526586 &  57650.86 &   349 &      3414 &     -0.08 &    4.16 &     2.153 \\
   J20303207+6526586 &  57651.75 &   337 &      3398 &     -0.05 &    4.17 &     2.016 \\
   J20303207+6526586 &  57673.72 &   361 &      3432 &     -0.04 &    4.17 &     2.240 \\
   J20303207+6526586 &  57674.80 &   316 &      3432 &     -0.05 &    4.19 &     2.199 \\
   J20303207+6526586 &  57675.69 &   328 &      3374 &     -0.04 &    4.22 &     2.275 \\
   J20303207+6526586 &  57676.69 &   367 &      3401 &     -0.06 &    4.22 &     2.465 \\
   J20303207+6526586 &  57677.75 &   328 &      3419 &     -0.05 &    4.20 &     2.455 \\
   J20303207+6526586 &  57678.76 &   294 &      3412 &     -0.06 &    4.20 &     2.175 \\
   J20303207+6526586 &  57680.79 &   360 &      3427 &     -0.05 &    4.16 &     2.443 \\
   J20303207+6526586 &  57682.79 &   369 &      3422 &     -0.06 &    4.18 &     2.243 \\
   J20414744+4938482 &  57673.78 &    53 &      3673 &      0.22 &    4.17 &         - \\
   J20523304-1658289 &  56907.73 &   407 &      3140 &      0.00 &    4.01 &     2.084 \\
   J20523304-1658289 &  56912.91 &   324 &      3148 &     -0.04 &    4.08 &     2.142 \\
   J20564659-1026534 &  57353.70 &   543 &      3437 &      0.10 &    3.91 &     2.068 \\
   J20564659-1026534 &  57500.12 &   212 &      3522 &      0.13 &    3.97 &     2.478 \\
   J21015865-0619070 &  57232.13 &   207 &      3411 &      0.10 &    3.98 &     2.099 \\
   J21015865-0619070 &  57263.97 &   256 &      3490 &      0.09 &    3.89 &     2.033 \\
   J21015865-0619070 &  57284.82 &   234 &      3463 &      0.07 &    3.94 &     2.508 \\
   J21015865-0619070 &  57227.07 &   278 &      3475 &      0.11 &    3.91 &     2.042 \\
   J21293671+1738353 &  57607.95 &   193 &      2259 &      0.01 &    4.07 &     2.731 \\
   J21293671+1738353 &  57652.77 &   198 &      1239 &     -0.19 &    8.99 &         - \\
   J21293671+1738353 &  57652.81 &   196 &      1148 &     -0.24 &    9.22 &     1.685 \\
   J21513828+5917383 &  57607.97 &   197 &      3230 &      0.21 &    3.79 &     2.078 \\
   J21513828+5917383 &  57651.95 &   286 &      3190 &      0.25 &    3.78 &     1.984 \\
   J22004701+7949254 &  57674.85 &    75 &      3712 &      0.07 &    4.24 &         - \\
   J22021026+0124006 &  57682.83 &   237 &      3848 &      0.28 &    4.27 &     2.617 \\
   J22022935-3704512 &  56909.83 &   330 &      3206 &     -0.06 &    3.97 &     2.284 \\
   J22022935-3704512 &  57226.97 &   307 &      3282 &     -0.05 &    3.99 &     2.122 \\
   J22245593+5200190 &  57673.86 &   100 &      3196 &     -0.27 &    5.26 &     2.600 \\
   J22270871+7751579 &  57673.80 &    74 &      3482 &     -0.08 &    4.53 &     1.464 \\
   J22270871+7751579 &  57677.87 &   128 &      2963 &      0.02 &    4.38 &     1.859 \\
   J22465311-0707272 &  57554.11 &   126 &      3894 &      0.65 &    4.61 &         - \\
   J22523963+7504190 &  57673.85 &    87 &      3320 &      0.17 &    3.89 &     1.782 \\
   J22524980+6629578 &  57611.94 &   171 &      3116 &      1.16 &    5.89 &         - \\
   J22524980+6629578 &  57680.82 &   263 &      3087 &      1.21 &    5.77 &         - \\
   J22531672-1415489 &  56883.89 &   273 &      3138 &      0.17 &    3.87 &     2.075 \\
   J22531672-1415489 &  56904.05 &   382 &      3123 &      0.14 &    3.88 &     2.082 \\
   J22554384-3022392 &  57232.10 &   115 &      3984 &      0.30 &    4.28 &         - \\
   J22554384-3022392 &  57200.12 &   117 &      3915 &      0.36 &    4.26 &     1.475 \\
   J23213752+1717284 &  56887.13 &   304 &      3069 &      0.20 &    3.79 &     1.826 \\
   J23213752+1717284 &  56971.87 &   382 &      3121 &      0.19 &    3.82 &     2.082 \\
   J23380819-1614100 &  57227.11 &   282 &      3491 &     -0.23 &    4.04 &     2.208 \\
   J23380819-1614100 &  57233.10 &   286 &      3484 &     -0.22 &    4.04 &     2.068 \\
   J23415498+4410407 &  57610.12 &   195 &      3075 &      0.04 &    4.36 &     2.244 \\
   J23415498+4410407 &  57652.07 &   202 &      3039 &      0.07 &    4.34 &     2.504 \\
   J23430628+3632132 &  56907.00 &   391 &      3093 &     -0.06 &    4.73 &     2.428 \\
   J23430628+3632132 &  57607.01 &   270 &      3133 &     -0.07 &    4.74 &     2.420 \\
   J23430628+3632132 &  57608.95 &   239 &    -32768 &         - &    4.74 &     2.344 \\
   J23430628+3632132 &  57611.12 &   241 &      3121 &     -0.04 &    4.73 &     2.052 \\
   J23430628+3632132 &  57613.13 &   243 &    -32768 &         - &    4.70 &     2.291 \\
   J23430628+3632132 &  57614.02 &   239 &    -32768 &         - &    4.70 &     2.191 \\
   J23430628+3632132 &  57615.98 &   290 &      3120 &     -0.05 &    4.71 &     2.367 \\
   J23430628+3632132 &  57646.06 &   238 &      3204 &     -0.08 &    4.55 &     2.320 \\
   J23430628+3632132 &  57649.93 &   253 &      3159 &     -0.03 &    4.60 &     2.305 \\
   J23430628+3632132 &  57650.90 &   247 &      3168 &     -0.02 &    4.56 &     2.389 \\
   J23430628+3632132 &  57651.82 &   243 &      3166 &     -0.02 &    4.54 &     2.372 \\
   J23430628+3632132 &  57652.78 &   247 &      3181 &     -0.08 &    4.56 &     2.199 \\
   J23430628+3632132 &  57653.91 &   245 &    -32768 &         - &    4.52 &     2.250 \\
   J23430628+3632132 &  57678.96 &   195 &      3113 &     -0.00 &    4.74 &     2.381 \\
   J23430628+3632132 &  57678.99 &   201 &      3171 &     -0.07 &    4.71 &     2.354 \\
   J23430628+3632132 &  57680.89 &   147 &      3222 &      0.00 &    4.80 &     2.528 \\
   J23430628+3632132 &  57680.92 &   196 &      3132 &     -0.04 &    4.71 &     2.379 \\
   J23430628+3632132 &  57681.97 &   249 &      3143 &     -0.07 &    4.70 &     2.432 \\
   J23430628+3632132 &  57682.84 &   248 &      3114 &     -0.06 &    4.71 &     2.541 \\
   J23430628+3632132 &  57230.12 &   390 &      3096 &     -0.04 &    4.55 &     2.343 \\
   J23583264+0739304 &  57227.09 &   290 &      3334 &      0.08 &    4.07 &     2.380 \\
   J23583264+0739304 &  57232.11 &   251 &      3354 &      0.05 &    4.09 &     2.914 \\
   J00182256+4401222 &  53547.13 &   312 &      3539 &     -0.29 &    4.19 &     2.018 \\
   J00182256+4401222 &  53546.12 &   441 &      3534 &     -0.32 &    4.21 &     2.210 \\
   J00182256+4401222 &  53952.07 &  1899 &      3521 &     -0.31 &    4.19 &     2.160 \\
   J00182256+4401222 &  28664.16 &  1471 &      3548 &     -0.32 &    4.11 &     2.277 \\
   J00243478+3002295 &  56551.96 &   148 &    -32768 &         - &    9.85 &     7.091 \\
   J00243478+3002295 &  56548.09 &   139 &    -32768 &         - &    9.94 &     5.326 \\
   J00243478+3002295 &  56559.84 &   148 &    -32768 &         - &    9.89 &     7.187 \\
   J00243478+3002295 &  56560.88 &   169 &    -32768 &         - &    9.69 &     6.496 \\
   J00243478+3002295 &  56555.80 &   135 &    -32768 &         - &    9.62 &     7.368 \\
   J01031971+6221557 &  54374.01 &   184 &    -32768 &         - &    0.00 &     0.000 \\
   J01031971+6221557 &  54754.04 &   169 &    -32768 &         - &   10.23 &     5.485 \\
   J01031971+6221557 &  54756.84 &   134 &    -32768 &         - &   12.17 &         - \\
   J01031971+6221557 &  54753.81 &   179 &    -32768 &         - &   12.01 &         - \\
   J01031971+6221557 &  54753.86 &   190 &    -32768 &         - &   11.01 &     6.981 \\
   J01031971+6221557 &  54753.95 &   165 &    -32768 &         - &   10.16 &     6.300 \\
   J01031971+6221557 &  54756.95 &    74 &    -32768 &         - &   12.58 &         - \\
   J01031971+6221557 &  54759.77 &   195 &    -32768 &         - &   11.01 &     6.090 \\
   J01031971+6221557 &  54759.84 &   169 &    -32768 &         - &   11.54 &     5.965 \\
   J01031971+6221557 &  54759.93 &   161 &    -32768 &         - &   11.65 &     6.798 \\
   J01031971+6221557 &  54760.02 &   172 &    -32768 &         - &   10.70 &     5.997 \\
   J01031971+6221557 &  53956.08 &   166 &    -32768 &         - &   10.76 &     5.918 \\
   J01031971+6221557 &  54371.97 &   182 &    -32768 &         - &   11.18 &     6.025 \\
   J01031971+6221557 &  54376.04 &   187 &    -32768 &         - &   11.57 &     5.922 \\
   J01031971+6221557 &  54377.04 &   209 &    -32768 &         - &   11.56 &     7.696 \\
   J01031971+6221557 &  53955.09 &   142 &    -32768 &         - &   10.88 &         - \\
   J01031971+6221557 &  53960.09 &   133 &    -32768 &         - &   10.68 &     6.350 \\
   J01031971+6221557 &  53957.08 &   145 &    -32768 &         - &   10.73 &     7.051 \\
   J01031971+6221557 &  53958.09 &    51 &      2907 &      1.02 &    4.78 &         - \\
   J01031971+6221557 &  54375.94 &   187 &    -32768 &         - &   11.75 &     7.015 \\
   J01031971+6221557 &  54376.94 &   208 &    -32768 &         - &   11.31 &     6.620 \\
   J01031971+6221557 &  53953.13 &   126 &    -32768 &         - &   14.61 &     5.862 \\
   J01031971+6221557 &  53959.09 &   152 &    -32768 &         - &   10.63 &     7.165 \\
   J01031971+6221557 &  54374.94 &   174 &    -32768 &         - &   12.12 &     6.507 \\
   J01031971+6221557 &  54375.82 &   168 &    -32768 &         - &   10.26 &     5.494 \\
   J01031971+6221557 &  54376.81 &   173 &    -32768 &         - &    9.92 &     5.805 \\
   J01390120-1757026 &  56556.95 &   376 &    -32768 &         - &   19.06 &         - \\
   J01390120-1757026 &  56556.98 &   353 &    -32768 &         - &   18.96 &         - \\
   J01390120-1757026 &  56556.93 &   312 &    -32768 &         - &   22.81 &         - \\
   J01390120-1757026 &  56559.93 &   292 &    -32768 &         - &   23.56 &         - \\
   J01390120-1757026 &  56559.98 &   303 &    -32768 &         - &   24.43 &         - \\
   J01390120-1757026 &  56560.05 &   292 &    -32768 &         - &   23.01 &         - \\
   J01390120-1757026 &  56560.10 &   243 &    -32768 &         - &   22.21 &         - \\
   J01390120-1757026 &  56557.08 &   338 &    -32768 &         - &   19.21 &         - \\
   J01390120-1757026 &  56557.05 &   337 &    -32768 &         - &   19.12 &         - \\
   J01390120-1757026 &  56557.03 &   286 &    -32768 &         - &   24.24 &         - \\
   J01390120-1757026 &  56557.11 &   294 &    -32768 &         - &   21.47 &         - \\
   J01390120-1757026 &  56557.00 &   284 &    -32768 &         - &   24.08 &         - \\
   J02001278+1303112 &  54373.93 &   322 &    -32768 &         - &    5.65 &     2.903 \\
   J02001278+1303112 &  54371.93 &   284 &    -32768 &         - &    5.61 &     2.951 \\
   J02001278+1303112 &  54375.90 &   304 &    -32768 &         - &    5.66 &     2.925 \\
   J02001278+1303112 &  54375.02 &   312 &    -32768 &         - &    5.67 &     3.093 \\
   J02001278+1303112 &  54376.90 &   316 &    -32768 &         - &    5.68 &     3.009 \\
   J02001278+1303112 &  54376.14 &   270 &    -32768 &         - &    5.72 &     2.871 \\
   J02001278+1303112 &  54377.13 &   300 &    -32768 &         - &    5.60 &     3.197 \\
   J02272924+3058246 &  56199.89 &   181 &      3688 &      1.08 &    5.22 &     1.241 \\
   J03392972+2458028 &  54373.04 &   159 &      3276 &     -0.12 &    4.79 &     2.477 \\
   J03392972+2458028 &  54373.07 &   159 &      3248 &     -0.13 &    4.80 &     2.417 \\
   J03392972+2458028 &  54373.10 &   174 &      3267 &     -0.09 &    4.77 &     2.093 \\
   J03392972+2458028 &  54373.12 &   176 &      3239 &     -0.12 &    4.76 &     2.751 \\
   J04302527+3951000 &  56529.08 &   216 &    -32768 &         - &   11.09 &     7.048 \\
   J04302527+3951000 &  56528.09 &   233 &    -32768 &         - &   10.69 &     6.710 \\
   J04302527+3951000 &  56530.09 &   165 &    -32768 &         - &   10.99 &     7.153 \\
   J04302527+3951000 &  56531.08 &   230 &    -32768 &         - &   10.36 &     6.800 \\
   J04302527+3951000 &  56532.05 &   225 &    -32768 &         - &   10.71 &     6.142 \\
   J04302527+3951000 &  56527.07 &   224 &    -32768 &         - &   10.77 &     7.762 \\
   J06544902+3316058 &  57475.80 &   271 &      3362 &      0.02 &    3.93 &         - \\
   J06544902+3316058 &  57324.98 &   258 &      3369 &     -0.06 &    3.89 &         - \\
   J06544902+3316058 &  56917.15 &   272 &      3346 &      0.02 &    3.85 &     2.150 \\
   J06544902+3316058 &  57012.07 &   235 &      3347 &     -0.01 &    3.94 &     2.274 \\
   J06544902+3316058 &  57012.07 &   234 &      3335 &     -0.03 &    3.94 &     2.113 \\
   J06544902+3316058 &  57014.12 &   257 &      3336 &     -0.02 &    3.92 &     2.071 \\
   J06544902+3316058 &  57037.05 &   235 &      3375 &     -0.02 &    3.91 &     2.096 \\
   J06544902+3316058 &  56915.14 &   280 &      3355 &      0.00 &    3.85 &     2.116 \\
   J06544902+3316058 &  56915.15 &   278 &      3323 &      0.02 &    3.88 &     2.015 \\
   J06544902+3316058 &  56917.14 &   257 &      3341 &      0.01 &    3.84 &     2.092 \\
   J06544902+3316058 &  56973.07 &   280 &      3326 &     -0.03 &    3.87 &     2.126 \\
   J06544902+3316058 &  57013.05 &   265 &      3323 &      0.01 &    3.92 &     2.096 \\
   J06544902+3316058 &  57021.09 &   258 &      3341 &      0.00 &    3.92 &     2.334 \\
   J06544902+3316058 &  57031.08 &   268 &      3387 &      0.02 &    3.89 &     1.980 \\
   J07100180+3831457 &  56619.88 &   567 &    -32768 &         - &    4.73 &     2.620 \\
   J07100180+3831457 &  56614.12 &   644 &      2261 &      0.05 &    4.47 &     2.291 \\
   J07100180+3831457 &  56616.09 &   615 &    -32768 &         - &    4.98 &     2.370 \\
   J07100180+3831457 &  56623.05 &   605 &    -32768 &         - &    4.78 &     1.717 \\
   J07343745+3152102 &  55931.81 &   678 &       984 &     -0.09 &   43.13 &     7.472 \\
   J07343745+3152102 &  55933.81 &   702 &      1000 &     -0.09 &   21.13 &     3.818 \\
   J07343745+3152102 &  55933.96 &   657 &      1006 &     -0.09 &   20.61 &         - \\
   J07343745+3152102 &  55934.76 &   719 &       999 &     -0.09 &   20.83 &         - \\
   J07343745+3152102 &  55935.80 &   726 &      1012 &     -0.11 &   19.84 &         - \\
   J07343745+3152102 &  55936.84 &   718 &      1010 &     -0.09 &   20.18 &         - \\
   J07343745+3152102 &  55937.09 &   640 &       961 &     -0.10 &   55.16 &         - \\
   J07343745+3152102 &  55937.93 &   607 &    -32768 &         - &   33.40 &         - \\
   J07343745+3152102 &  55938.08 &   695 &      1025 &     -0.08 &   20.01 &         - \\
   J07343745+3152102 &  55941.08 &    97 &      1199 &     -0.07 &   20.05 &         - \\
   J07343745+3152102 &  55930.80 &   711 &      1010 &     -0.10 &   19.36 &         - \\
   J07343745+3152102 &  55930.94 &   662 &      1004 &     -0.09 &   20.49 &         - \\
   J07343745+3152102 &  55931.04 &   551 &      1010 &     -0.09 &   32.57 &         - \\
   J07343745+3152102 &  55931.95 &   576 &      1012 &     -0.10 &   20.14 &         - \\
   J07343745+3152102 &  55932.12 &   603 &      1027 &     -0.11 &   20.22 &         - \\
   J07343745+3152102 &  55932.84 &   645 &      1005 &     -0.09 &   20.46 &         - \\
   J07343745+3152102 &  55932.92 &   637 &      1024 &     -0.09 &   20.21 &         - \\
   J07343745+3152102 &  55933.07 &   466 &    -32768 &         - &   28.84 &         - \\
   J07343745+3152102 &  55934.09 &   661 &      1040 &     -0.08 &   19.46 &         - \\
   J07343745+3152102 &  55934.95 &   712 &      1007 &     -0.08 &   20.28 &         - \\
   J07343745+3152102 &  55935.09 &   580 &      1019 &     -0.08 &   28.24 &         - \\
   J07343745+3152102 &  55935.97 &   722 &      1005 &     -0.09 &   21.01 &         - \\
   J07343745+3152102 &  55936.05 &   721 &      1009 &     -0.10 &   20.27 &         - \\
   J07343745+3152102 &  55936.98 &   694 &      1027 &     -0.09 &   20.12 &         - \\
   J07343745+3152102 &  55937.85 &   700 &       994 &     -0.10 &   20.81 &         - \\
   J07343745+3152102 &  55938.79 &   650 &       966 &     -0.09 &   49.01 &         - \\
   J07343745+3152102 &  55938.96 &   690 &      1026 &     -0.09 &   19.28 &         - \\
   J07343745+3152102 &  55939.09 &   641 &       999 &     -0.10 &   20.49 &         - \\
   J07343745+3152102 &  55940.80 &   495 &    -32768 &         - &   26.40 &         - \\
   J07343745+3152102 &  55941.10 &   228 &      1029 &     -0.10 &   20.57 &         - \\
   J07343745+3152102 &  55941.12 &   109 &      1113 &     -0.10 &   20.82 &         - \\
   J07343745+3152102 &  55942.00 &   242 &    -32768 &         - &   31.80 &         - \\
   J07343745+3152102 &  55942.04 &   375 &       995 &     -0.09 &   37.68 &         - \\
   J07343745+3152102 &  55942.05 &   467 &       975 &     -0.09 &   53.96 &         - \\
   J07343745+3152102 &  55943.08 &   650 &       993 &     -0.09 &   19.79 &         - \\
   J07343745+3152102 &  55944.07 &   576 &      1001 &     -0.09 &   36.88 &         - \\
   J07444018+0333089 &  53773.94 &   326 &    -32768 &         - &    7.83 &         - \\
   J07444018+0333089 &  54485.93 &   263 &    -32768 &         - &    7.41 &     3.935 \\
   J07444018+0333089 &  53748.92 &   199 &    -32768 &         - &    7.89 &     3.342 \\
   J08115757+0846220 &  53748.95 &   153 &      3398 &     -0.51 &    5.13 &     2.610 \\
   J08294949+2646348 &  54483.86 &   117 &    -32768 &         - &   10.08 &     6.112 \\
   J08294949+2646348 &  54164.94 &   165 &    -32768 &         - &   10.27 &     6.737 \\
   J08294949+2646348 &  54165.93 &   116 &    -32768 &         - &   10.58 &         - \\
   J08294949+2646348 &  54166.91 &   127 &    -32768 &         - &   10.16 &     5.563 \\
   J08294949+2646348 &  54486.04 &   151 &    -32768 &         - &   10.24 &     6.284 \\
   J08294949+2646348 &  54163.93 &   161 &    -32768 &         - &   10.12 &     6.149 \\
   J08294949+2646348 &  54487.98 &   143 &    -32768 &         - &   10.37 &     5.389 \\
   J08294949+2646348 &  54878.75 &   184 &    -32768 &         - &   10.33 &     6.117 \\
   J08294949+2646348 &  54878.88 &   179 &    -32768 &         - &   10.41 &     6.459 \\
   J08294949+2646348 &  54875.88 &   121 &    -32768 &         - &   10.71 &     7.501 \\
   J08294949+2646348 &  54876.74 &   101 &    -32768 &         - &   10.52 &     5.855 \\
   J08294949+2646348 &  54876.87 &   128 &    -32768 &         - &   10.60 &         - \\
   J08294949+2646348 &  54876.99 &   102 &    -32768 &         - &   10.44 &         - \\
   J08294949+2646348 &  54877.74 &   158 &    -32768 &         - &   10.37 &     7.204 \\
   J08294949+2646348 &  54877.87 &   167 &    -32768 &         - &   10.36 &         - \\
   J08294949+2646348 &  54878.01 &   154 &    -32768 &         - &   10.38 &     6.992 \\
   J08294949+2646348 &  54879.00 &   170 &    -32768 &         - &   10.50 &     6.839 \\
   J08294949+2646348 &  54838.88 &    54 &    -32768 &         - &   10.54 &     4.642 \\
   J08294949+2646348 &  54487.04 &   156 &    -32768 &         - &   10.96 &     6.349 \\
   J08294949+2646348 &  54839.16 &    18 &      3469 &      1.12 &   11.84 &         - \\
   J08294949+2646348 &  54485.04 &    90 &    -32768 &         - &   10.13 &     5.923 \\
   J08294949+2646348 &  54161.93 &   157 &    -32768 &         - &   10.21 &         - \\
   J08294949+2646348 &  54484.86 &   136 &    -32768 &         - &   10.13 &         - \\
   J08294949+2646348 &  54486.86 &   132 &    -32768 &         - &   10.32 &     6.521 \\
   J08294949+2646348 &  54839.06 &     6 &      1377 &     -0.50 &    1.14 &219849.641 \\
   J08313759+1923395 &  55932.96 &   495 &    -32768 &         - &    8.09 &     5.250 \\
   J08313759+1923395 &  55933.11 &   452 &    -32768 &         - &    7.49 &         - \\
   J08313759+1923395 &  55941.03 &   274 &    -32768 &         - &    7.30 &     6.266 \\
   J08313759+1923395 &  55942.82 &   365 &    -32768 &         - &    7.61 &     6.882 \\
   J08313759+1923395 &  55930.90 &   495 &    -32768 &         - &    6.97 &     4.093 \\
   J08313759+1923395 &  55931.13 &   419 &    -32768 &         - &    6.99 &     6.593 \\
   J08313759+1923395 &  55931.98 &   514 &    -32768 &         - &    7.02 &     4.439 \\
   J08313759+1923395 &  55934.12 &   479 &    -32768 &         - &    7.31 &     3.648 \\
   J08313759+1923395 &  55935.05 &   517 &    -32768 &         - &    6.87 &     4.310 \\
   J08313759+1923395 &  55935.83 &   520 &    -32768 &         - &   21.76 &     6.418 \\
   J08313759+1923395 &  55936.08 &   503 &    -32768 &         - &    7.08 &     4.987 \\
   J08313759+1923395 &  55937.89 &   506 &    -32768 &         - &    6.91 &         - \\
   J08313759+1923395 &  55938.11 &   490 &    -32768 &         - &    7.03 &     4.475 \\
   J08313759+1923395 &  55939.00 &   503 &    -32768 &         - &    7.06 &     4.396 \\
   J08313759+1923395 &  55939.12 &   462 &    -32768 &         - &    7.07 &     9.272 \\
   J08313759+1923395 &  55940.89 &   469 &    -32768 &         - &    7.14 &     4.179 \\
   J08313759+1923395 &  55941.85 &   247 &    -32768 &         - &    7.04 &         - \\
   J08313759+1923395 &  55942.87 &   404 &    -32768 &         - &    7.19 &     3.962 \\
   J08313759+1923395 &  55943.12 &   459 &    -32768 &         - &    7.03 &     3.399 \\
   J08313759+1923395 &  55933.91 &   513 &    -32768 &         - &    6.97 &     8.845 \\
   J09142298+5241125 &  54275.77 &   468 &      3859 &      0.35 &    4.57 &         - \\
   J10121768-0344441 &  57030.10 &   297 &      3609 &      0.20 &    4.19 &     2.006 \\
   J10164599-1157412 &  54169.96 &   161 &      1032 &     -0.09 &   43.34 &         - \\
   J10182870-3150029 &  54170.00 &   169 &      1056 &     -0.06 &   44.80 &         - \\
   J10193634+1952122 &  53748.88 &   316 &    -32768 &         - &    6.03 &         - \\
   J10193634+1952122 &  54276.77 &   801 &    -32768 &         - &    5.75 &         - \\
   J10193634+1952122 &  53897.80 &   797 &    -32768 &         - &    5.86 &         - \\
   J10193634+1952122 &  53896.81 &   757 &    -32768 &         - &    5.83 &         - \\
   J10193634+1952122 &  53780.06 &   387 &    -32768 &         - &    5.97 &         - \\
   J10193634+1952122 &  53895.80 &   481 &    -32768 &         - &    5.90 &         - \\
   J10193634+1952122 &  53747.08 &   273 &    -32768 &         - &    6.01 &         - \\
   J10193634+1952122 &  53898.78 &   754 &    -32768 &         - &    5.87 &         - \\
   J10481258-1120082 &  54878.05 &   122 &    -32768 &         - &    7.71 &         - \\
   J10481258-1120082 &  54875.92 &   103 &    -32768 &         - &    7.97 &         - \\
   J10481258-1120082 &  54876.91 &    81 &    -32768 &         - &    8.19 &         - \\
   J10481258-1120082 &  54877.04 &    65 &    -32768 &         - &    8.19 &         - \\
   J10481258-1120082 &  54877.92 &   138 &    -32768 &         - &    7.67 &         - \\
   J10481258-1120082 &  54878.92 &   150 &    -32768 &         - &    7.61 &         - \\
   J10481258-1120082 &  54879.05 &   134 &    -32768 &         - &    7.71 &     3.953 \\
   J10481258-1120082 &  54879.91 &   160 &    -32768 &         - &    7.75 &         - \\
   J10481258-1120082 &  54880.04 &   150 &    -32768 &         - &    7.78 &     3.734 \\
   J10481258-1120082 &  27270.65 &    20 &      2727 &      0.74 &    6.28 &         - \\
   J10481258-1120082 &  54545.84 &   158 &    -32768 &         - &    7.55 &         - \\
   J10481258-1120082 &  54548.00 &   156 &    -32768 &         - &    7.61 &         - \\
   J10481258-1120082 &  54548.91 &   158 &    -32768 &         - &    7.58 &     3.604 \\
   J10481258-1120082 &  54550.81 &   153 &    -32768 &         - &    7.43 &     3.683 \\
   J10481258-1120082 &  54551.81 &   167 &    -32768 &         - &    7.54 &     3.817 \\
   J10481258-1120082 &  54552.91 &   149 &    -32768 &         - &    7.51 &     3.652 \\
   J10481258-1120082 &  54553.85 &   136 &    -32768 &         - &    7.39 &     3.382 \\
   J10481258-1120082 &  54546.93 &   160 &    -32768 &         - &    7.69 &     3.193 \\
   J10505201+0648292 &  53749.00 &   134 &      3108 &      0.03 &    4.06 &     1.605 \\
   J10562886+0700527 &  54548.87 &   324 &    -32768 &         - &    6.95 &         - \\
   J10562886+0700527 &  56827.75 &     5 &      1717 &     -0.23 &    0.77 &         - \\
   J10562886+0700527 &  54546.98 &   267 &    -32768 &         - &    7.05 &         - \\
   J10562886+0700527 &  54547.91 &   208 &    -32768 &         - &    7.07 &         - \\
   J10562886+0700527 &  54547.95 &   222 &    -32768 &         - &    7.04 &         - \\
   J11000432+2249592 &  27270.73 &   108 &    -32768 &         - &    6.20 &     3.953 \\
   J11015191-3442170 &  27271.17 &   173 &    -32768 &         - &    6.09 &     2.441 \\
   J11015191-3442170 &  54545.89 &   269 &    -32768 &         - &    6.02 &     3.173 \\
   J11015191-3442170 &  54545.94 &   272 &    -32768 &         - &    5.99 &     2.700 \\
   J11015191-3442170 &  54548.82 &   269 &    -32768 &         - &    6.18 &         - \\
   J11015191-3442170 &  54548.96 &   282 &    -32768 &         - &    6.19 &     3.141 \\
   J11015191-3442170 &  54551.86 &   273 &    -32768 &         - &    6.13 &     2.478 \\
   J11015191-3442170 &  54552.81 &   286 &    -32768 &         - &    6.02 &     2.882 \\
   J11015191-3442170 &  54552.95 &   249 &    -32768 &         - &    5.98 &     2.609 \\
   J11015191-3442170 &  54553.80 &   277 &    -32768 &         - &    5.94 &     2.271 \\
   J11015191-3442170 &  54553.90 &   183 &    -32768 &         - &    6.03 &     3.666 \\
   J11015191-3442170 &  54553.94 &   192 &    -32768 &         - &    6.05 &         - \\
   J11015191-3442170 &  55252.03 &   274 &    -32768 &         - &    6.46 &     3.648 \\
   J11015191-3442170 &  55258.01 &   172 &    -32768 &         - &    6.30 &         - \\
   J11015191-3442170 &  55962.01 &   299 &    -32768 &         - &    6.19 &     2.865 \\
   J11015191-3442170 &  55969.03 &   227 &    -32768 &         - &    6.22 &         - \\
   J11015191-3442170 &  55250.99 &   253 &    -32768 &         - &    6.38 &     3.332 \\
   J11015191-3442170 &  55252.95 &   260 &    -32768 &         - &    6.13 &     3.350 \\
   J11015191-3442170 &  55254.01 &   267 &    -32768 &         - &    6.13 &     2.330 \\
   J11015191-3442170 &  55256.02 &   255 &    -32768 &         - &    6.31 &         - \\
   J11015191-3442170 &  55257.00 &   233 &    -32768 &         - &    6.39 &     2.151 \\
   J11015191-3442170 &  55258.95 &   163 &    -32768 &         - &    6.32 &     2.722 \\
   J11015191-3442170 &  55260.00 &   229 &    -32768 &         - &    6.35 &     3.339 \\
   J11015191-3442170 &  55260.95 &   201 &    -32768 &         - &    6.24 &     3.218 \\
   J11015191-3442170 &  55262.97 &   230 &    -32768 &         - &    6.16 &     3.699 \\
   J11015191-3442170 &  55263.95 &   170 &    -32768 &         - &    6.22 &     3.707 \\
   J11015191-3442170 &  55957.98 &   282 &    -32768 &         - &    6.09 &     3.138 \\
   J11015191-3442170 &  55958.99 &   263 &    -32768 &         - &    5.93 &     2.886 \\
   J11015191-3442170 &  55960.03 &   263 &    -32768 &         - &    6.33 &     2.676 \\
   J11015191-3442170 &  55961.02 &   249 &    -32768 &         - &    6.27 &     2.858 \\
   J11015191-3442170 &  55964.96 &   239 &    -32768 &         - &    6.20 &     2.934 \\
   J11015191-3442170 &  55964.99 &   249 &    -32768 &         - &    6.12 &     2.938 \\
   J11015191-3442170 &  55966.97 &   247 &    -32768 &         - &    6.15 &     2.318 \\
   J11015191-3442170 &  55967.03 &   267 &    -32768 &         - &    6.33 &     3.221 \\
   J11015191-3442170 &  55968.04 &   289 &    -32768 &         - &    6.21 &     2.892 \\
   J11015191-3442170 &  55969.97 &   268 &    -32768 &         - &    6.17 &     2.956 \\
   J11015191-3442170 &  55971.04 &   232 &    -32768 &         - &    6.11 &     3.000 \\
   J11015191-3442170 &  55254.93 &   247 &    -32768 &         - &    6.21 &     3.749 \\
   J11015191-3442170 &  27271.22 &   192 &    -32768 &         - &    6.23 &     2.835 \\
   J11023832+2158017 &  53774.03 &   363 &      3660 &      0.23 &    4.78 &     1.803 \\
   J11023832+2158017 &  53781.15 &   265 &      3686 &      0.22 &    4.76 &         - \\
   J11023832+2158017 &  53748.90 &   189 &      3669 &      0.25 &    4.77 &     1.360 \\
   J11023832+2158017 &  54275.81 &   546 &      3685 &      0.22 &    4.77 &     2.413 \\
   J11023832+2158017 &  53748.10 &   349 &      3683 &      0.24 &    4.81 &     2.341 \\
   J11032023+3558117 &  57415.05 &   752 &      3543 &     -0.42 &    4.07 &     2.170 \\
   J11032023+3558117 &  57411.02 &   518 &      3546 &     -0.39 &    4.06 &     2.117 \\
   J11032023+3558117 &  57415.02 &   750 &      3531 &     -0.41 &    4.07 &     1.989 \\
   J11032023+3558117 &  57415.03 &   752 &      3531 &     -0.43 &    4.07 &     2.270 \\
   J11032023+3558117 &  57415.04 &   755 &      3544 &     -0.42 &    4.06 &     2.147 \\
   J11032023+3558117 &  57415.04 &   759 &      3542 &     -0.41 &    4.06 &     2.108 \\
   J11032023+3558117 &  57415.05 &   750 &      3540 &     -0.41 &    4.07 &     2.073 \\
   J11032023+3558117 &  57415.06 &  1221 &      3539 &     -0.43 &    4.07 &     2.003 \\
   J11032023+3558117 &  57415.00 &   748 &      3557 &     -0.41 &    4.07 &     2.112 \\
   J11052903+4331357 &  53749.02 &   332 &      3499 &     -0.36 &    4.35 &     1.919 \\
   J11053133+4331170 &  54165.01 &   162 &    -32768 &         - &   15.73 &     5.081 \\
   J11053133+4331170 &  54168.04 &   148 &    -32768 &         - &   16.30 &     4.814 \\
   J11053133+4331170 &  54487.11 &   139 &    -32768 &         - &   14.50 &     4.815 \\
   J11053133+4331170 &  54166.94 &   140 &    -32768 &         - &   15.67 &     5.403 \\
   J11053133+4331170 &  54483.93 &    79 &    -32768 &         - &   14.31 &     5.141 \\
   J11053133+4331170 &  54165.96 &    85 &    -32768 &         - &   15.40 &     4.092 \\
   J11053133+4331170 &  54486.11 &   121 &    -32768 &         - &   15.38 &     4.374 \\
   J11053133+4331170 &  54162.99 &   121 &    -32768 &         - &   15.50 &     4.138 \\
   J11053133+4331170 &  54163.97 &   162 &    -32768 &         - &   16.02 &     5.089 \\
   J11053133+4331170 &  54161.97 &   156 &    -32768 &         - &   14.85 &     4.391 \\
   J11053133+4331170 &  53773.97 &   114 &    -32768 &         - &  182.16 &     5.117 \\
   J11053133+4331170 &  53774.00 &   119 &    -32768 &         - &  179.76 &     1.021 \\
   J11053133+4331170 &  53898.74 &   134 &    -32768 &         - &   16.81 &     5.210 \\
   J11053133+4331170 &  53895.84 &    79 &    -32768 &         - &   17.04 &     5.319 \\
   J11053133+4331170 &  53896.84 &   134 &    -32768 &         - &   16.07 &     5.132 \\
   J11053133+4331170 &  53896.77 &   154 &    -32768 &         - &   17.03 &     5.189 \\
   J11053133+4331170 &  53897.83 &   140 &    -32768 &         - &   16.20 &     5.143 \\
   J11053133+4331170 &  53897.77 &   152 &    -32768 &         - &   16.94 &     4.880 \\
   J11053133+4331170 &  53895.77 &    94 &    -32768 &         - &   16.55 &     5.014 \\
   J11053133+4331170 &  53898.81 &   133 &    -32768 &         - &   17.10 &     5.361 \\
   J11053133+4331170 &  54484.92 &    72 &    -32768 &         - &   14.66 &     4.336 \\
   J11053133+4331170 &  54486.92 &   131 &    -32768 &         - &   14.69 &     4.428 \\
   J11053133+4331170 &  54845.98 &   158 &    -32768 &         - &   15.92 &         - \\
   J11053133+4331170 &  54844.04 &   123 &    -32768 &         - &   15.88 &         - \\
   J11053133+4331170 &  54843.01 &   125 &    -32768 &         - &   15.83 &         - \\
   J11053133+4331170 &  54843.11 &   121 &    -32768 &         - &   15.97 &     4.234 \\
   J11053133+4331170 &  54843.94 &   145 &    -32768 &         - &   15.95 &         - \\
   J11053133+4331170 &  54844.14 &   147 &    -32768 &         - &   15.83 &     3.905 \\
   J11053133+4331170 &  54844.94 &   146 &    -32768 &         - &   14.56 &     3.879 \\
   J11053133+4331170 &  54845.16 &   171 &    -32768 &         - &   14.62 &         - \\
   J11053133+4331170 &  54846.07 &   178 &    -32768 &         - &   15.41 &         - \\
   J11053133+4331170 &  54846.16 &   171 &    -32768 &         - &   14.98 &     5.285 \\
   J11053133+4331170 &  54845.09 &   160 &    -32768 &         - &   14.71 &         - \\
   J11115176+3332111 &  56677.14 &   224 &    -32768 &         - &    6.39 &     2.725 \\
   J11115176+3332111 &  56669.12 &   215 &    -32768 &         - &    6.44 &     2.378 \\
   J11115176+3332111 &  56678.09 &   206 &    -32768 &         - &    6.48 &     2.791 \\
   J11115176+3332111 &  56666.06 &   199 &    -32768 &         - &    7.45 &     3.213 \\
   J11115176+3332111 &  56667.14 &   181 &    -32768 &         - &    7.01 &         - \\
   J11115176+3332111 &  56668.16 &   202 &    -32768 &         - &    6.65 &     2.646 \\
   J11115176+3332111 &  56670.01 &   138 &    -32768 &         - &    6.55 &         - \\
   J11115176+3332111 &  56670.02 &   192 &    -32768 &         - &    6.45 &     2.828 \\
   J11115176+3332111 &  56672.07 &   179 &    -32768 &         - &    7.13 &     2.978 \\
   J11115176+3332111 &  56674.17 &   193 &    -32768 &         - &    7.48 &     3.479 \\
   J11115176+3332111 &  56675.14 &   213 &    -32768 &         - &    6.85 &         - \\
   J11115176+3332111 &  56679.09 &   222 &    -32768 &         - &    6.73 &     2.799 \\
   J11115176+3332111 &  56680.04 &   149 &    -32768 &         - &    7.44 &     3.366 \\
   J11200526+6550470 &  53568.76 &   690 &      3547 &     -0.47 &    4.33 &     1.448 \\
   J11220530-2446393 &  56344.89 &   419 &      2373 &      0.50 &   10.57 &     2.269 \\
   J11220530-2446393 &  56351.96 &   384 &      2310 &      0.45 &   10.30 &     1.134 \\
   J11220530-2446393 &  56352.10 &   169 &      2035 &      0.24 &   11.39 &     1.271 \\
   J11220530-2446393 &  56353.96 &   343 &      2293 &      0.45 &   10.28 &     1.493 \\
   J11220530-2446393 &  56343.95 &   372 &      2404 &      0.51 &   10.15 &     1.886 \\
   J11220530-2446393 &  56352.87 &   412 &      2183 &      0.35 &   10.85 &     2.903 \\
   J11220530-2446393 &  56354.09 &   328 &      2335 &      0.47 &   10.18 &     4.190 \\
   J11220530-2446393 &  56354.88 &   373 &      2184 &      0.37 &   10.73 &    87.106 \\
   J11220530-2446393 &  56355.04 &   227 &      2263 &      0.43 &   10.19 &     0.762 \\
   J11220530-2446393 &  56355.95 &   383 &      2341 &      0.49 &    9.97 &     3.485 \\
   J11220530-2446393 &  56356.09 &   340 &      2169 &      0.34 &   10.77 &     2.083 \\
   J11220530-2446393 &  56353.02 &   331 &      2225 &      0.40 &   10.70 &     2.961 \\
   J11220530-2446393 &  56345.09 &   395 &      2556 &      0.63 &    9.12 &     1.887 \\
   J11314655-4102473 &  56677.12 &   276 &    -32768 &         - &   14.18 &     3.787 \\
   J11314655-4102473 &  56680.05 &   227 &    -32768 &         - &   14.57 &   201.035 \\
   J11314655-4102473 &  56667.12 &   194 &    -32768 &         - &   14.19 &    10.931 \\
   J11314655-4102473 &  56668.09 &   271 &    -32768 &         - &   14.17 &    10.996 \\
   J11314655-4102473 &  56669.10 &   306 &    -32768 &         - &   14.11 &     6.317 \\
   J11314655-4102473 &  56670.04 &   233 &    -32768 &         - &   14.08 &     8.184 \\
   J11314655-4102473 &  56672.10 &   214 &    -32768 &         - &   14.34 &         - \\
   J11314655-4102473 &  56674.15 &   232 &    -32768 &         - &   14.43 &         - \\
   J11314655-4102473 &  56675.12 &   294 &    -32768 &         - &   14.42 &         - \\
   J11314655-4102473 &  56678.07 &   254 &    -32768 &         - &   14.13 &         - \\
   J11314655-4102473 &  56679.06 &   313 &    -32768 &         - &   14.58 &         - \\
   J11474143+7841283 &  53748.98 &   248 &      3229 &     -0.22 &    4.12 &         - \\
   J12100559-1504156 &  54165.05 &   151 &    -32768 &         - &   13.89 &         - \\
   J12141654+0037263 &  54166.97 &   148 &    -32768 &         - &    6.73 &         - \\
   J12141654+0037263 &  54164.01 &   175 &    -32768 &         - &    6.61 &         - \\
   J12141654+0037263 &  54165.99 &   154 &    -32768 &         - &    6.61 &         - \\
   J12141654+0037263 &  54488.01 &   170 &    -32768 &         - &    6.46 &         - \\
   J12141654+0037263 &  54163.02 &   124 &    -32768 &         - &    6.65 &         - \\
   J12141654+0037263 &  54162.01 &   158 &    -32768 &         - &    6.67 &         - \\
   J12141654+0037263 &  54485.01 &    89 &    -32768 &         - &    6.99 &         - \\
   J12141654+0037263 &  54487.01 &   140 &    -32768 &         - &    6.65 &         - \\
   J12141654+0037263 &  54486.01 &   157 &    -32768 &         - &    6.66 &         - \\
   J12185939+1107338 &  54165.08 &   165 &    -32768 &         - &   10.96 &         - \\
   J12185939+1107338 &  54164.04 &   182 &    -32768 &         - &   11.12 &         - \\
   J12185939+1107338 &  54488.09 &   155 &    -32768 &         - &   11.38 &         - \\
   J12185939+1107338 &  54163.05 &   121 &    -32768 &         - &   11.47 &         - \\
   J12185939+1107338 &  54841.16 &   191 &    -32768 &         - &   11.52 &         - \\
   J12185939+1107338 &  54840.01 &   202 &    -32768 &         - &   11.85 &         - \\
   J12185939+1107338 &  54840.10 &   195 &    -32768 &         - &   11.45 &         - \\
   J12185939+1107338 &  54840.16 &   172 &    -32768 &         - &   13.34 &         - \\
   J12185939+1107338 &  54841.02 &   174 &    -32768 &         - &   11.59 &     7.000 \\
   J12185939+1107338 &  54841.09 &   191 &    -32768 &         - &   11.37 &         - \\
   J12185939+1107338 &  54842.02 &   190 &    -32768 &         - &   11.85 &     8.406 \\
   J12185939+1107338 &  54842.09 &   188 &    -32768 &         - &   11.46 &     8.331 \\
   J12185939+1107338 &  54842.16 &   189 &    -32768 &         - &   11.37 &     7.974 \\
   J12185939+1107338 &  54167.00 &   161 &    -32768 &         - &   12.11 &     6.844 \\
   J12185939+1107338 &  54162.04 &   153 &    -32768 &         - &   11.26 &         - \\
   J12185939+1107338 &  54166.02 &   140 &    -32768 &         - &   11.29 &     9.424 \\
   J12185939+1107338 &  54484.98 &    71 &    -32768 &         - &   12.59 &         - \\
   J12185939+1107338 &  54485.98 &   157 &    -32768 &         - &   11.82 &    10.233 \\
   J12185939+1107338 &  54486.98 &   132 &    -32768 &         - &   11.92 &     8.710 \\
   J12185939+1107338 &  54487.14 &   151 &    -32768 &         - &   11.19 &         - \\
   J12185939+1107338 &  54486.14 &   157 &    -32768 &         - &   11.37 &     9.050 \\
   J12573935+3513194 &  54550.08 &   156 &    -32768 &         - &   23.00 &     0.914 \\
   J12573935+3513194 &  54550.87 &   137 &    -32768 &         - &   22.78 &         - \\
   J12573935+3513194 &  54551.98 &   134 &    -32768 &         - &   22.81 &    10.278 \\
   J12573935+3513194 &  54549.80 &   144 &    -32768 &         - &   22.78 &     9.131 \\
   J12573935+3513194 &  54549.83 &   147 &    -32768 &         - &   22.39 &     1.410 \\
   J12573935+3513194 &  54549.85 &   148 &    -32768 &         - &   22.36 &     0.912 \\
   J12573935+3513194 &  54549.90 &   145 &    -32768 &         - &   22.63 &     0.847 \\
   J12573935+3513194 &  54549.95 &   148 &    -32768 &         - &   22.60 &     2.716 \\
   J12573935+3513194 &  54549.98 &   152 &    -32768 &         - &   22.30 &     1.134 \\
   J12573935+3513194 &  54550.00 &   153 &    -32768 &         - &   22.33 &     3.689 \\
   J12573935+3513194 &  54550.03 &   152 &    -32768 &         - &   22.28 &     2.582 \\
   J12573935+3513194 &  54550.05 &   153 &    -32768 &         - &   21.65 &     0.700 \\
   J12573935+3513194 &  54550.89 &   140 &    -32768 &         - &   22.64 &     3.255 \\
   J12573935+3513194 &  54550.92 &   147 &    -32768 &         - &   22.50 &         - \\
   J12573935+3513194 &  54550.95 &   142 &    -32768 &         - &   22.92 &         - \\
   J12573935+3513194 &  54550.97 &   143 &    -32768 &         - &   22.89 &     1.059 \\
   J12573935+3513194 &  54550.99 &   149 &    -32768 &         - &   22.53 &         - \\
   J12573935+3513194 &  54551.02 &   152 &    -32768 &         - &   22.52 &     7.519 \\
   J12573935+3513194 &  54551.05 &   151 &    -32768 &         - &   22.48 &     2.762 \\
   J12573935+3513194 &  54551.07 &   143 &    -32768 &         - &   22.64 &         - \\
   J12573935+3513194 &  54551.10 &   146 &    -32768 &         - &   22.62 &         - \\
   J12573935+3513194 &  54551.91 &   142 &    -32768 &         - &   22.84 &         - \\
   J12573935+3513194 &  54551.94 &   144 &    -32768 &         - &   22.59 &         - \\
   J12573935+3513194 &  54551.96 &   146 &    -32768 &         - &   22.80 &         - \\
   J12573935+3513194 &  54552.01 &   138 &    -32768 &         - &   22.82 &         - \\
   J12573935+3513194 &  54552.03 &   137 &    -32768 &         - &   22.77 &         - \\
   J12573935+3513194 &  54552.06 &   143 &    -32768 &         - &   22.92 &         - \\
   J12573935+3513194 &  54552.08 &   139 &    -32768 &         - &   22.64 &         - \\
   J12573935+3513194 &  54552.11 &   136 &    -32768 &         - &   22.47 &         - \\
   J12573935+3513194 &  54552.13 &   117 &    -32768 &         - &   22.74 &         - \\
   J12573935+3513194 &  54553.09 &   138 &    -32768 &         - &   22.53 &         - \\
   J12573935+3513194 &  54549.88 &   148 &    -32768 &         - &   22.66 &         - \\
   J12573935+3513194 &  54549.93 &   148 &    -32768 &         - &   22.44 &         - \\
   J13003350+0541081 &  56352.97 &   210 &    -32768 &         - &   11.98 &         - \\
   J13003350+0541081 &  56354.06 &   195 &    -32768 &         - &   11.79 &         - \\
   J13003350+0541081 &  56355.06 &   176 &    -32768 &         - &   11.76 &         - \\
   J13003350+0541081 &  56355.96 &   216 &    -32768 &         - &   11.97 &         - \\
   J13003350+0541081 &  56356.11 &   194 &    -32768 &         - &   11.76 &         - \\
   J13004666+1222325 &  53780.16 &   179 &    -32768 &         - &    8.20 &         - \\
   J13004666+1222325 &  53781.17 &   306 &    -32768 &         - &    8.47 &         - \\
   J13004666+1222325 &  53774.05 &   362 &    -32768 &         - &    8.21 &         - \\
   J13004666+1222325 &  53896.87 &   236 &    -32768 &         - &    8.37 &         - \\
   J13142039+1320011 &  56429.75 &    92 &    -32768 &         - &   28.73 &         - \\
   J13142039+1320011 &  56429.79 &    94 &    -32768 &         - &   28.98 &         - \\
   J13142039+1320011 &  56429.84 &    72 &    -32768 &         - &   28.66 &         - \\
   J13142039+1320011 &  56429.88 &    69 &    -32768 &         - &   28.30 &         - \\
   J13295979+1022376 &  57032.16 &   293 &      3673 &      0.00 &    4.11 &         - \\
   J13314666+2916368 &  56428.75 &   340 &    -32768 &         - &   48.00 &         - \\
   J13314666+2916368 &  56428.82 &   345 &    -32768 &         - &   48.07 &         - \\
   J13314666+2916368 &  56428.88 &   342 &    -32768 &         - &   48.57 &         - \\
   J13314666+2916368 &  56429.05 &   242 &    -32768 &         - &   46.92 &         - \\
   J13454354+1453317 &  57033.14 &   433 &      3616 &     -0.30 &    4.04 &         - \\
   J14010324-0239180 &  57032.16 &   262 &      3678 &     -0.04 &    4.07 &     2.313 \\
   J15215291+2058394 &  54275.90 &   914 &    -32768 &         - &    6.02 &     3.166 \\
   J16334161-0933116 &  56884.74 &   321 &      3809 &      0.46 &    5.25 &     2.037 \\
   J16360563+0848491 &  56434.88 &   162 &      3082 &     -0.06 &    4.64 &     2.442 \\
   J16360563+0848491 &  56465.99 &   145 &      3045 &     -0.05 &    4.69 &     2.754 \\
   J16360563+0848491 &  56459.99 &   174 &      3102 &     -0.01 &    4.60 &         - \\
   J16360563+0848491 &  56470.02 &   160 &      3053 &     -0.06 &    4.78 &     2.733 \\
   J16360563+0848491 &  56471.98 &   140 &      3161 &     -0.07 &    4.67 &     2.477 \\
   J16400599+0042188 &  56464.78 &   170 &    -32768 &         - &   19.31 &     0.742 \\
   J16400599+0042188 &  56458.77 &   187 &    -32768 &         - &   19.34 &         - \\
   J16400599+0042188 &  56460.93 &   163 &    -32768 &         - &   19.18 &         - \\
   J16400599+0042188 &  56465.86 &   162 &    -32768 &         - &   19.33 &         - \\
   J16400599+0042188 &  56468.85 &   176 &    -32768 &         - &   19.26 &         - \\
   J16400599+0042188 &  56472.02 &   149 &    -32768 &         - &   19.17 &    11.060 \\
   J16402068+6736046 &  56459.75 &   124 &    -32768 &         - &   12.30 &         - \\
   J16402068+6736046 &  56460.97 &   118 &    -32768 &         - &   12.16 &         - \\
   J16402068+6736046 &  56458.81 &   130 &    -32768 &         - &   11.88 &         - \\
   J16402068+6736046 &  56458.99 &   124 &    -32768 &         - &   12.04 &     6.052 \\
   J16402068+6736046 &  56459.93 &   124 &    -32768 &         - &   12.06 &     5.904 \\
   J16402068+6736046 &  56460.77 &   122 &    -32768 &         - &   12.03 &     5.608 \\
   J16552880-0820103 &  56520.86 &   820 &    -32768 &         - &    6.14 &     3.426 \\
   J16552880-0820103 &  56521.73 &   876 &    -32768 &         - &   13.15 &     1.177 \\
   J16552880-0820103 &  56522.82 &   720 &    -32768 &         - &   14.87 &     3.018 \\
   J16552880-0820103 &  53950.79 &  1192 &      2286 &     -0.09 &    6.76 &     5.099 \\
   J16553529-0823401 &  54954.88 &   104 &    -32768 &         - &   10.25 &     4.878 \\
   J16553529-0823401 &  54956.89 &    95 &    -32768 &         - &   10.34 &     5.236 \\
   J16553529-0823401 &  54956.99 &    98 &    -32768 &         - &   10.06 &     5.238 \\
   J16553529-0823401 &  54955.09 &   107 &    -32768 &         - &   10.27 &         - \\
   J16553529-0823401 &  54956.00 &    93 &    -32768 &         - &   10.44 &         - \\
   J16553529-0823401 &  54956.10 &    98 &    -32768 &         - &   10.48 &         - \\
   J16553529-0823401 &  54957.10 &   103 &    -32768 &         - &   10.10 &         - \\
   J16553529-0823401 &  54954.98 &   106 &    -32768 &         - &   10.52 &         - \\
   J16553529-0823401 &  54955.89 &    85 &    -32768 &         - &    9.84 &         - \\
   J18073292-1557464 &  54645.88 &   125 &    -32768 &         - &    6.42 &     3.426 \\
   J18073292-1557464 &  54643.02 &   199 &    -32768 &         - &    6.13 &     2.994 \\
   J18073292-1557464 &  54646.94 &   161 &    -32768 &         - &    6.22 &     2.764 \\
   J18073292-1557464 &  54649.94 &     0 &    -32768 &         - &    6.28 &     2.647 \\
   J18073292-1557464 &  54650.91 &   187 &    -32768 &         - &    6.13 &     2.951 \\
   J18073292-1557464 &  54651.84 &   193 &    -32768 &         - &    6.15 &     2.752 \\
   J18073292-1557464 &  54652.85 &   200 &         0 &      0.00 &    6.22 &     3.618 \\
   J18073292-1557464 &  54653.82 &   208 &         0 &      0.00 &    6.19 &         - \\
   J18073292-1557464 &  54654.88 &   188 &         0 &      0.00 &    6.08 &         - \\
   J18073292-1557464 &  54656.95 &   191 &         0 &      0.00 &    6.14 &         - \\
   J18073292-1557464 &  54655.84 &   193 &         0 &      0.00 &    6.09 &     3.529 \\
   J18073292-1557464 &  54645.92 &   120 &    -32768 &         - &    6.45 &         - \\
   J18185725+6611332 &  56462.78 &   193 &    -32768 &         - &   11.59 &     8.658 \\
   J18185725+6611332 &  56458.96 &   211 &    -32768 &         - &   11.82 &     7.150 \\
   J18185725+6611332 &  56459.79 &   204 &    -32768 &         - &   11.55 &     7.492 \\
   J18185725+6611332 &  56464.83 &   209 &    -32768 &         - &   11.31 &     8.015 \\
   J18424498+1354168 &  56523.87 &   254 &    -32768 &         - &    5.69 &     2.897 \\
   J18424498+1354168 &  56525.77 &   268 &    -32768 &         - &    5.52 &         - \\
   J18424498+1354168 &  56521.76 &   256 &    -32768 &         - &    5.47 &     2.730 \\
   J18424498+1354168 &  56527.92 &   246 &    -32768 &         - &    5.53 &         - \\
   J18424498+1354168 &  56529.94 &   111 &    -32768 &         - &    5.78 &     2.559 \\
   J18424498+1354168 &  56531.82 &   247 &    -32768 &         - &    5.65 &     2.607 \\
   J18424688+5937374 &  53601.75 &   505 &      3275 &     -0.30 &    4.17 &     2.245 \\
   J18552740+0824090 &  56766.97 &   407 &    -32768 &         - &    5.15 &     5.620 \\
   J18552740+0824090 &  56763.07 &   535 &    -32768 &         - &   17.39 &     4.236 \\
   J18552740+0824090 &  56763.99 &   558 &    -32768 &         - &    6.27 &     3.734 \\
   J18552740+0824090 &  56767.12 &   429 &    -32768 &         - &    5.18 &     4.051 \\
   J18552740+0824090 &  56772.10 &   609 &    -32768 &         - &    5.27 &     2.386 \\
   J18552740+0824090 &  56757.02 &   575 &    -32768 &         - &    5.38 &     3.295 \\
   J18552740+0824090 &  56757.13 &   622 &    -32768 &         - &    5.33 &     4.481 \\
   J18552740+0824090 &  56758.01 &   523 &    -32768 &         - &    7.01 &     4.548 \\
   J18552740+0824090 &  56758.12 &   533 &    -32768 &         - &    5.79 &     2.966 \\
   J18552740+0824090 &  56759.00 &   591 &    -32768 &         - &   12.32 &     1.688 \\
   J18552740+0824090 &  56759.12 &   614 &    -32768 &         - &   13.68 &     1.710 \\
   J18552740+0824090 &  28380.25 &   333 &    -32768 &         - &    5.47 &     2.179 \\
   J18552740+0824090 &  28380.28 &   275 &    -32768 &         - &    5.43 &     2.706 \\
   J18552740+0824090 &  56761.01 &   512 &    -32768 &         - &    5.27 &         - \\
   J18552740+0824090 &  56762.12 &   426 &    -32768 &         - &    5.29 &         - \\
   J18552740+0824090 &  56764.12 &   637 &    -32768 &         - &    5.33 &         - \\
   J18552740+0824090 &  56764.97 &   533 &    -32768 &         - &    5.73 &     1.946 \\
   J18552740+0824090 &  56765.12 &   616 &    -32768 &         - &    5.27 &     4.870 \\
   J18552740+0824090 &  56765.98 &   326 &    -32768 &         - &    5.11 &     2.050 \\
   J18552740+0824090 &  56766.13 &   486 &    -32768 &         - &    5.06 &     1.866 \\
   J18552740+0824090 &  56769.00 &   232 &    -32768 &         - &    8.58 &     6.632 \\
   J18552740+0824090 &  56769.03 &   374 &    -32768 &         - &    8.91 &     6.585 \\
   J18552740+0824090 &  56770.00 &   466 &    -32768 &         - &    6.06 &     2.340 \\
   J18552740+0824090 &  56770.12 &   543 &    -32768 &         - &    5.74 &     2.389 \\
   J18552740+0824090 &  56771.98 &   621 &    -32768 &         - &    5.28 &         - \\
   J18552740+0824090 &  56763.13 &   555 &    -32768 &         - &   16.81 &     3.842 \\
   J18552740+0824090 &  56762.00 &   402 &    -32768 &         - &    5.31 &     2.657 \\
   J18552740+0824090 &  54275.99 &   777 &    -32768 &         - &    6.19 &     2.088 \\
   J19165762+0509021 &  55013.95 &    68 &    -32768 &         - &    8.12 &     4.780 \\
   J19165762+0509021 &  55015.09 &    77 &    -32768 &         - &    8.85 &     4.833 \\
   J19165762+0509021 &  55014.01 &    76 &    -32768 &         - &    8.25 &     4.016 \\
   J19165762+0509021 &  55014.06 &    76 &    -32768 &         - &    8.38 &     5.072 \\
   J19165762+0509021 &  55014.95 &    72 &    -32768 &         - &    8.19 &         - \\
   J19165762+0509021 &  55015.93 &    75 &    -32768 &         - &    8.67 &         - \\
   J19165762+0509021 &  55016.04 &    73 &    -32768 &         - &    8.35 &     4.141 \\
   J19165762+0509021 &  55016.09 &    74 &    -32768 &         - &    8.13 &     4.214 \\
   J19165762+0509021 &  55015.00 &    71 &    -32768 &         - &    8.19 &     3.700 \\
   J19510930+4628598 &  53633.73 &   107 &    -32768 &         - &   16.05 &   852.728 \\
   J19510930+4628598 &  53632.73 &   108 &    -32768 &         - &   14.80 &     4.964 \\
   J19510930+4628598 &  56521.98 &   205 &    -32768 &         - &   14.96 &         - \\
   J19510930+4628598 &  56522.88 &   179 &    -32768 &         - &   15.23 &     4.995 \\
   J19510930+4628598 &  56521.82 &   223 &    -32768 &         - &   15.06 &   540.240 \\
   J19510930+4628598 &  56522.77 &   192 &    -32768 &         - &   15.07 &     6.573 \\
   J19535508+4424550 &  54699.99 &   177 &    -32768 &         - &    8.30 &     5.406 \\
   J19535508+4424550 &  54700.98 &   152 &    -32768 &         - &    8.16 &     4.730 \\
   J19535508+4424550 &  54701.02 &   144 &    -32768 &         - &    8.19 &     5.185 \\
   J19535508+4424550 &  53955.95 &   194 &    -32768 &         - &    7.97 &     5.089 \\
   J19535508+4424550 &  54373.88 &   195 &    -32768 &         - &    7.90 &     5.188 \\
   J19535443+4424541 &  56522.73 &   243 &    -32768 &         - &   15.63 &         - \\
   J19535443+4424541 &  56522.79 &   221 &    -32768 &         - &   15.73 &     9.587 \\
   J19535443+4424541 &  56522.86 &   234 &    -32768 &         - &   15.74 &    10.212 \\
   J19535443+4424541 &  56522.91 &   240 &    -32768 &         - &   15.66 &         - \\
   J19535508+4424550 &  54700.86 &   155 &    -32768 &         - &    8.32 &         - \\
   J19535508+4424550 &  54699.87 &   193 &    -32768 &         - &    8.14 &         - \\
   J19535508+4424550 &  54698.84 &   193 &         0 &      0.00 &    8.09 &         - \\
   J19535508+4424550 &  54700.73 &   154 &    -32768 &         - &    8.36 &         - \\
   J19535508+4424550 &  54698.74 &   190 &    -32768 &         - &    8.28 &         - \\
   J19535508+4424550 &  54698.99 &   173 &         0 &      0.00 &    8.09 &         - \\
   J19535508+4424550 &  54699.74 &   194 &    -32768 &         - &    8.02 &         - \\
   J19535508+4424550 &  53952.96 &   172 &    -32768 &         - &    8.38 &         - \\
   J19535508+4424550 &  53958.95 &   188 &    -32768 &         - &    8.10 &         - \\
   J19535508+4424550 &  53959.96 &   162 &    -32768 &         - &    8.56 &         - \\
   J19535508+4424550 &  54375.86 &   179 &    -32768 &         - &    8.19 &         - \\
   J19535508+4424550 &  53957.95 &   184 &    -32768 &         - &    8.30 &         - \\
   J19535508+4424550 &  54376.86 &   214 &    -32768 &         - &    7.83 &         - \\
   J19535508+4424550 &  53956.96 &   179 &    -32768 &         - &    8.22 &         - \\
   J19535508+4424550 &  54376.72 &   224 &    -32768 &         - &    7.84 &     5.294 \\
   J19535508+4424550 &  54375.72 &   203 &    -32768 &         - &    8.16 &     5.111 \\
   J19535508+4424550 &  54374.86 &   197 &    -32768 &         - &    7.96 &         - \\
   J20294834+0941202 &  56560.84 &   241 &    -32768 &         - &   21.23 &     0.979 \\
   J20294834+0941202 &  56547.82 &   225 &    -32768 &         - &   21.09 &     3.256 \\
   J20294834+0941202 &  56548.89 &   250 &    -32768 &         - &   21.33 &     1.707 \\
   J20294834+0941202 &  56549.73 &   256 &    -32768 &         - &   21.04 &         - \\
   J20294834+0941202 &  56552.00 &   115 &    -32768 &         - &   20.90 &         - \\
   J20450949-3120266 &  53567.95 &  1072 &      2465 &      0.20 &    7.48 &         - \\
   J20450949-3120266 &  53568.00 &   919 &      2482 &      0.21 &    7.46 &     4.664 \\
   J20450949-3120266 &  53568.91 &   984 &    -32768 &         - &    7.46 &     4.430 \\
   J20450949-3120266 &  53569.00 &  1002 &    -32768 &         - &    7.48 &     4.565 \\
   J20450949-3120266 &  53949.89 &   779 &    -32768 &         - &    7.57 &     4.766 \\
   J20450949-3120266 &  53949.94 &   480 &    -32768 &         - &    7.55 &     4.340 \\
   J20450949-3120266 &  53949.97 &   604 &    -32768 &         - &    7.55 &     4.060 \\
   J20450949-3120266 &  53950.02 &   904 &    -32768 &         - &    7.53 &     5.014 \\
   J20450949-3120266 &  53950.92 &   819 &    -32768 &         - &    7.37 &     5.091 \\
   J20450949-3120266 &  53950.96 &   620 &    -32768 &         - &    7.37 &     4.080 \\
   J20450949-3120266 &  53950.99 &   710 &    -32768 &         - &    7.38 &     5.238 \\
   J20450949-3120266 &  53896.10 &   858 &    -32768 &         - &    7.66 &     4.249 \\
   J20450949-3120266 &  53896.12 &   857 &    -32768 &         - &    7.69 &     4.994 \\
   J20560274-1710538 &  56463.12 &   205 &      1804 &      0.13 &   10.15 &    22.336 \\
   J20560274-1710538 &  56462.96 &   206 &      1772 &      0.13 &   10.17 &     0.813 \\
   J20560274-1710538 &  56467.91 &   232 &      1778 &      0.12 &   10.10 &     0.755 \\
   J20560274-1710538 &  56458.94 &   224 &      1773 &      0.13 &   10.19 &     6.695 \\
   J20560274-1710538 &  56459.97 &   221 &      1759 &      0.10 &   10.18 &     0.954 \\
   J20560274-1710538 &  56460.12 &   222 &      1755 &      0.10 &   10.21 &         - \\
   J20560274-1710538 &  56460.90 &   217 &      1787 &      0.14 &   10.11 &         - \\
   J20560274-1710538 &  56461.11 &   200 &      1794 &      0.16 &   10.12 &         - \\
   J20560274-1710538 &  56464.94 &   225 &      1752 &      0.13 &   10.21 &         - \\
   J20560274-1710538 &  56465.10 &   221 &      1725 &      0.12 &   10.29 &         - \\
   J20560274-1710538 &  56465.93 &   208 &      1701 &      0.08 &   10.34 &   231.367 \\
   J20560274-1710538 &  56466.11 &   194 &      1722 &      0.12 &   10.34 &     6.444 \\
   J20560274-1710538 &  56468.10 &   210 &      1783 &      0.13 &   10.16 &     2.435 \\
   J20560274-1710538 &  56471.95 &   218 &      1744 &      0.10 &   10.27 &     1.256 \\
   J20560274-1710538 &  56472.12 &   201 &      1764 &      0.13 &   10.22 &     7.966 \\
   J20560274-1710538 &  56473.91 &   220 &      1776 &      0.12 &   10.18 &     3.186 \\
   J21000529+4004136 &  56519.74 &   527 &    -32768 &         - &    6.80 &     4.572 \\
   J21000529+4004136 &  56517.75 &   644 &    -32768 &         - &    6.93 &     3.443 \\
   J21000529+4004136 &  56524.04 &   534 &    -32768 &         - &    7.24 &     3.337 \\
   J21000529+4004136 &  56525.00 &   567 &    -32768 &         - &    6.97 &     2.735 \\
   J21000529+4004136 &  56518.00 &   537 &    -32768 &         - &    6.93 &     2.927 \\
   J21000529+4004136 &  56518.99 &   324 &    -32768 &         - &    7.82 &     4.505 \\
   J21000529+4004136 &  56519.02 &   329 &    -32768 &         - &    7.58 &     4.044 \\
   J21000529+4004136 &  56520.00 &   564 &    -32768 &         - &    6.99 &         - \\
   J21000529+4004136 &  56520.90 &   542 &    -32768 &         - &    7.14 &         - \\
   J21000529+4004136 &  56521.79 &   605 &    -32768 &         - &    7.54 &         - \\
   J21000529+4004136 &  56522.00 &   584 &    -32768 &         - &    7.72 &         - \\
   J21000529+4004136 &  56522.96 &   569 &    -32768 &         - &    6.78 &         - \\
   J21000529+4004136 &  56523.84 &   590 &    -32768 &         - &    9.11 &         - \\
   J21000529+4004136 &  56525.90 &   616 &    -32768 &         - &    6.79 &         - \\
   J21000529+4004136 &  56527.03 &   548 &    -32768 &         - &    8.57 &         - \\
   J21000529+4004136 &  56527.96 &   587 &    -32768 &         - &    6.86 &         - \\
   J21000529+4004136 &  56528.96 &   542 &    -32768 &         - &    7.07 &         - \\
   J21000529+4004136 &  56529.97 &   327 &    -32768 &         - &    7.83 &         - \\
   J21000529+4004136 &  56530.95 &   566 &    -32768 &         - &    6.96 &         - \\
   J21000529+4004136 &  56531.74 &   661 &    -32768 &         - &    8.76 &         - \\
   J21000529+4004136 &  56531.92 &   604 &    -32768 &         - &    7.62 &         - \\
   J21000529+4004136 &  56519.05 &   452 &    -32768 &         - &    7.35 &         - \\
   J21000529+4004136 &  56525.74 &   580 &    -32768 &         - &    6.97 &         - \\
   J21000529+4004136 &  54276.98 &   750 &    -32768 &         - &    6.74 &     5.521 \\
   J21374019+0137137 &  54702.80 &   114 &    -32768 &         - &   28.61 &     0.605 \\
   J21374019+0137137 &  54702.82 &   114 &    -32768 &         - &   28.24 &     5.586 \\
   J21374019+0137137 &  54702.86 &   118 &    -32768 &         - &   27.54 &     7.712 \\
   J21374019+0137137 &  54702.77 &   114 &    -32768 &         - &   27.85 &     2.984 \\
   J21374019+0137137 &  54702.84 &   118 &    -32768 &         - &   27.60 &     1.485 \\
   J21374019+0137137 &  54702.88 &   117 &    -32768 &         - &   26.88 &     0.519 \\
   J21374019+0137137 &  54702.75 &   110 &    -32768 &         - &   27.40 &     0.494 \\
   J21374019+0137137 &  55411.91 &    98 &    -32768 &         - &   25.69 &     3.712 \\
   J21374019+0137137 &  55409.91 &   106 &    -32768 &         - &   25.98 &     0.944 \\
   J21374019+0137137 &  55410.91 &   104 &    -32768 &         - &   27.71 &     0.555 \\
   J21374019+0137137 &  55413.89 &    73 &    -32768 &         - &   26.70 &     2.876 \\
   J21374019+0137137 &  54702.90 &   125 &    -32768 &         - &   26.27 &     1.604 \\
   J21374019+0137137 &  54702.92 &   119 &    -32768 &         - &   26.98 &    22.204 \\
   J21374019+0137137 &  54702.95 &   120 &    -32768 &         - &   27.29 &     1.750 \\
   J21374019+0137137 &  54702.96 &   119 &    -32768 &         - &   27.24 &     3.099 \\
   J21374019+0137137 &  54702.98 &   116 &    -32768 &         - &   27.61 &     0.789 \\
   J21374019+0137137 &  54703.00 &   119 &    -32768 &         - &   27.41 &     3.130 \\
   J21374019+0137137 &  54703.03 &   115 &    -32768 &         - &   27.19 &     1.216 \\
   J21374019+0137137 &  54703.05 &   110 &    -32768 &         - &   26.63 &         - \\
   J21374019+0137137 &  54372.88 &   145 &    -32768 &         - &   27.42 &    12.565 \\
   J22011310+2818248 &  53604.03 &   184 &    -32768 &         - &   21.96 &     6.695 \\
   J22011310+2818248 &  53604.08 &   170 &    -32768 &         - &   21.72 &     0.418 \\
   J22011310+2818248 &  53603.92 &   156 &    -32768 &         - &   21.96 &     1.143 \\
   J22011310+2818248 &  53603.94 &   150 &    -32768 &         - &   21.84 &         - \\
   J22011310+2818248 &  53603.96 &   152 &    -32768 &         - &   21.67 &         - \\
   J22011310+2818248 &  53603.98 &   166 &    -32768 &         - &   21.43 &         - \\
   J22011310+2818248 &  53603.99 &   188 &    -32768 &         - &   21.57 &         - \\
   J22011310+2818248 &  53604.01 &   189 &    -32768 &         - &   21.73 &         - \\
   J22011310+2818248 &  53604.05 &   178 &    -32768 &         - &   21.65 &         - \\
   J22011310+2818248 &  53604.06 &   175 &    -32768 &         - &   21.53 &         - \\
   J22011310+2818248 &  53604.10 &   165 &    -32768 &         - &   21.92 &         - \\
   J22011310+2818248 &  53604.12 &   156 &    -32768 &         - &   22.11 &         - \\
   J22011310+2818248 &  53604.13 &   146 &    -32768 &         - &   22.02 &         - \\
   J22011310+2818248 &  53603.78 &   178 &    -32768 &         - &   21.91 &         - \\
   J22011310+2818248 &  53603.76 &   166 &    -32768 &         - &   22.14 &         - \\
   J22011310+2818248 &  53603.81 &   171 &    -32768 &         - &   21.81 &         - \\
   J22011310+2818248 &  53603.83 &   169 &    -32768 &         - &   21.85 &         - \\
   J22011310+2818248 &  53603.88 &   163 &    -32768 &         - &   22.00 &         - \\
   J22011310+2818248 &  53603.91 &   170 &    -32768 &         - &   22.73 &         - \\
   J22011310+2818248 &  53603.74 &   159 &    -32768 &         - &   22.08 &         - \\
   J22011310+2818248 &  53603.80 &   173 &    -32768 &         - &   21.80 &         - \\
   J22011310+2818248 &  53603.85 &   171 &    -32768 &         - &   21.80 &         - \\
   J22011310+2818248 &  53603.87 &   161 &    -32768 &         - &   21.95 &         - \\
   J22011310+2818248 &  55079.07 &   165 &    -32768 &         - &   21.83 &         - \\
   J22011310+2818248 &  55080.74 &   201 &    -32768 &         - &   21.61 &         - \\
   J22011310+2818248 &  55081.03 &   211 &    -32768 &         - &   22.04 &         - \\
   J22011310+2818248 &  55078.79 &   191 &    -32768 &         - &   22.00 &         - \\
   J22011310+2818248 &  55078.84 &   187 &    -32768 &         - &   22.02 &         - \\
   J22011310+2818248 &  55078.86 &   180 &    -32768 &         - &   21.36 &         - \\
   J22011310+2818248 &  55078.89 &   189 &    -32768 &         - &   21.25 &         - \\
   J22011310+2818248 &  55078.96 &   180 &    -32768 &         - &   21.49 &         - \\
   J22011310+2818248 &  55079.74 &   204 &    -32768 &         - &   21.71 &         - \\
   J22011310+2818248 &  55079.84 &   219 &    -32768 &         - &   21.56 &         - \\
   J22011310+2818248 &  55079.93 &   202 &    -32768 &         - &   21.78 &         - \\
   J22011310+2818248 &  55079.98 &   199 &    -32768 &         - &   21.47 &         - \\
   J22011310+2818248 &  55080.05 &   196 &    -32768 &         - &   21.50 &         - \\
   J22011310+2818248 &  55080.79 &   210 &    -32768 &         - &   21.55 &         - \\
   J22011310+2818248 &  55080.84 &   209 &    -32768 &         - &   22.07 &         - \\
   J22011310+2818248 &  55080.88 &   205 &    -32768 &         - &   21.77 &         - \\
   J22011310+2818248 &  55080.93 &   208 &    -32768 &         - &   21.25 &         - \\
   J22011310+2818248 &  55080.97 &   212 &    -32768 &         - &   21.86 &         - \\
   J22011310+2818248 &  55078.94 &   171 &    -32768 &         - &   21.47 &         - \\
   J22011310+2818248 &  55079.88 &   203 &    -32768 &         - &   21.64 &         - \\
   J22011310+2818248 &  53605.82 &   146 &    -32768 &         - &   22.03 &         - \\
   J22011310+2818248 &  53605.91 &   179 &    -32768 &         - &   22.12 &         - \\
   J22011310+2818248 &  53605.73 &   176 &    -32768 &         - &   21.71 &         - \\
   J22011310+2818248 &  53606.11 &   144 &    -32768 &         - &   22.05 &         - \\
   J22011310+2818248 &  55079.02 &   176 &    -32768 &         - &   21.64 &         - \\
   J22011310+2818248 &  55080.01 &   203 &    -32768 &         - &   21.29 &         - \\
   J22011310+2818248 &  55080.99 &   215 &    -32768 &         - &   21.64 &         - \\
   J22011310+2818248 &  53605.75 &   176 &    -32768 &         - &   21.67 &         - \\
   J22011310+2818248 &  53605.77 &   181 &    -32768 &         - &   21.73 &         - \\
   J22011310+2818248 &  53605.79 &   180 &    -32768 &         - &   21.76 &         - \\
   J22011310+2818248 &  53605.80 &   160 &    -32768 &         - &   22.13 &         - \\
   J22011310+2818248 &  53605.84 &   149 &    -32768 &         - &   21.77 &         - \\
   J22011310+2818248 &  53605.86 &   173 &    -32768 &         - &   21.77 &         - \\
   J22011310+2818248 &  53605.88 &   164 &    -32768 &         - &   23.17 &         - \\
   J22011310+2818248 &  53605.89 &   173 &    -32768 &         - &   22.55 &         - \\
   J22011310+2818248 &  53605.93 &   181 &    -32768 &         - &   21.95 &         - \\
   J22011310+2818248 &  53605.95 &   181 &    -32768 &         - &   21.89 &         - \\
   J22011310+2818248 &  53605.96 &   179 &    -32768 &         - &   21.87 &         - \\
   J22011310+2818248 &  53605.98 &   178 &    -32768 &         - &   22.08 &         - \\
   J22011310+2818248 &  53606.02 &   171 &    -32768 &         - &   22.06 &         - \\
   J22011310+2818248 &  53606.04 &   162 &    -32768 &         - &   21.98 &         - \\
   J22011310+2818248 &  53606.05 &   167 &    -32768 &         - &   21.78 &         - \\
   J22011310+2818248 &  53606.12 &   133 &    -32768 &         - &   21.90 &         - \\
   J22011310+2818248 &  53953.03 &   190 &    -32768 &         - &   21.64 &         - \\
   J22011310+2818248 &  53953.05 &   190 &    -32768 &         - &   21.37 &         - \\
   J22011310+2818248 &  55079.79 &   214 &    -32768 &         - &   21.29 &         - \\
   J22011310+2818248 &  53606.00 &   172 &    -32768 &         - &   22.16 &         - \\
   J22011310+2818248 &  53606.07 &   166 &    -32768 &         - &   21.74 &         - \\
   J22011310+2818248 &  53606.09 &   156 &    -32768 &         - &   21.90 &         - \\
   J22011310+2818248 &  53602.05 &   169 &    -32768 &         - &   21.71 &         - \\
   J22011310+2818248 &  53602.08 &   171 &    -32768 &         - &   21.81 &         - \\
   J22011310+2818248 &  53601.78 &   177 &    -32768 &         - &   22.03 &         - \\
   J22011310+2818248 &  53601.80 &   180 &    -32768 &         - &   22.06 &         - \\
   J22011310+2818248 &  53601.81 &   174 &    -32768 &         - &   21.86 &         - \\
   J22011310+2818248 &  53601.83 &   170 &    -32768 &         - &   21.56 &         - \\
   J22011310+2818248 &  53601.85 &   133 &    -32768 &         - &    0.00 &         - \\
   J22011310+2818248 &  53601.87 &   129 &    -32768 &         - &    0.00 &         - \\
   J22011310+2818248 &  53601.90 &     7 &      2387 &      1.50 &    5.36 &         - \\
   J22011310+2818248 &  53601.91 &     8 &      2717 &      0.90 &     NaN &         - \\
   J22011310+2818248 &  53601.94 &   104 &    -32768 &         - &   22.03 &         - \\
   J22011310+2818248 &  53601.95 &   104 &    -32768 &         - &   22.17 &         - \\
   J22011310+2818248 &  53601.97 &   159 &    -32768 &         - &   22.05 &         - \\
   J22011310+2818248 &  53601.98 &   183 &    -32768 &         - &   22.06 &         - \\
   J22011310+2818248 &  53602.00 &   182 &    -32768 &         - &   22.05 &         - \\
   J22011310+2818248 &  53602.02 &   178 &    -32768 &         - &   22.11 &         - \\
   J22011310+2818248 &  53602.04 &   173 &    -32768 &         - &   21.52 &         - \\
   J22011310+2818248 &  53602.09 &   166 &    -32768 &         - &   21.94 &         - \\
   J22011310+2818248 &  53602.11 &   159 &    -32768 &         - &   21.93 &         - \\
   J22011310+2818248 &  53602.13 &   150 &    -32768 &         - &   21.92 &         - \\
   J22011310+2818248 &  53955.85 &   173 &    -32768 &         - &   21.98 &         - \\
   J22011310+2818248 &  53955.87 &   192 &    -32768 &         - &   21.72 &         - \\
   J22011310+2818248 &  53956.02 &   204 &    -32768 &         - &   21.77 &         - \\
   J22011310+2818248 &  53956.03 &   204 &    -32768 &         - &   21.86 &         - \\
   J22011310+2818248 &  53956.82 &   195 &    -32768 &         - &   21.57 &         - \\
   J22011310+2818248 &  53956.84 &   199 &    -32768 &         - &   21.73 &         - \\
   J22011310+2818248 &  53955.02 &   199 &    -32768 &         - &   21.69 &         - \\
   J22011310+2818248 &  53955.04 &   197 &    -32768 &         - &   21.81 &         - \\
   J22011310+2818248 &  53959.04 &   222 &    -32768 &         - &   21.61 &         - \\
   J22011310+2818248 &  53959.02 &   223 &    -32768 &         - &   21.77 &     1.011 \\
   J22011310+2818248 &  53960.03 &   218 &    -32768 &         - &   21.74 &     1.078 \\
   J22011310+2818248 &  53960.05 &   215 &    -32768 &         - &   21.66 &         - \\
   J22011310+2818248 &  53958.02 &   220 &    -32768 &         - &   21.96 &         - \\
   J22011310+2818248 &  53958.04 &   207 &    -32768 &         - &   21.91 &         - \\
   J22011310+2818248 &  53952.91 &   183 &    -32768 &         - &   21.58 &         - \\
   J22011310+2818248 &  53952.93 &   190 &    -32768 &         - &   21.49 &         - \\
   J22011310+2818248 &  53957.02 &   194 &    -32768 &         - &   21.75 &         - \\
   J22011310+2818248 &  53957.04 &   195 &    -32768 &         - &   21.54 &         - \\
   J22011310+2818248 &  53957.84 &   222 &    -32768 &         - &   21.68 &         - \\
   J22011310+2818248 &  53957.86 &   227 &    -32768 &         - &   21.72 &         - \\
   J22384559-2037160 &  56904.03 &   630 &    -32768 &         - &    6.15 &         - \\
   J22384559-2037160 &  56907.84 &   707 &    -32768 &         - &    6.60 &         - \\
   J22384559-2037160 &  56908.81 &   456 &      2471 &     -0.02 &    6.16 &         - \\
   J22384559-2037160 &  56908.83 &   403 &      2469 &     -0.03 &    6.17 &         - \\
   J22384559-2037160 &  56911.80 &   665 &    -32768 &         - &    8.96 &         - \\
   J22384559-2037160 &  56916.99 &   632 &      2502 &     -0.00 &    6.16 &         - \\
   J22384559-2037160 &  53568.95 &   944 &    -32768 &         - &    6.16 &         - \\
   J22384559-2037160 &  56903.86 &   697 &    -32768 &         - &    8.06 &         - \\
   J22384559-2037160 &  56904.79 &   657 &      2496 &     -0.03 &    6.21 &         - \\
   J22384559-2037160 &  56904.89 &   701 &      2455 &     -0.01 &    6.23 &         - \\
   J22384559-2037160 &  56905.91 &   623 &    -32768 &         - &    7.42 &         - \\
   J22384559-2037160 &  56906.93 &   661 &    -32768 &         - &    5.93 &         - \\
   J22384559-2037160 &  56907.03 &   675 &    -32768 &         - &    6.00 &         - \\
   J22384559-2037160 &  56907.98 &   634 &    -32768 &         - &    6.53 &         - \\
   J22384559-2037160 &  56908.96 &   555 &      2463 &     -0.02 &    6.20 &         - \\
   J22384559-2037160 &  56908.98 &   523 &      2465 &     -0.02 &    6.21 &         - \\
   J22384559-2037160 &  56909.80 &   679 &    -32768 &         - &    7.95 &         - \\
   J22384559-2037160 &  56909.95 &   650 &    -32768 &         - &    9.58 &         - \\
   J22384559-2037160 &  56910.80 &   315 &      2497 &      0.03 &    5.96 &         - \\
   J22384559-2037160 &  56910.82 &   461 &      2536 &      0.01 &    5.96 &         - \\
   J22384559-2037160 &  56910.84 &   226 &      2509 &      0.06 &    5.93 &         - \\
   J22384559-2037160 &  56910.92 &   687 &      2566 &      0.06 &    5.94 &         - \\
   J22384559-2037160 &  56911.94 &   608 &    -32768 &         - &    7.48 &         - \\
   J22384559-2037160 &  56911.95 &   599 &    -32768 &         - &    8.17 &     6.619 \\
   J22384559-2037160 &  56912.80 &   586 &      2489 &     -0.01 &    6.16 &     3.407 \\
   J22384559-2037160 &  56912.97 &   600 &      2497 &     -0.01 &    6.17 &     3.250 \\
   J22384559-2037160 &  56906.03 &   617 &    -32768 &         - &    6.25 &     3.999 \\
   J22464980+4420030 &  53956.05 &   511 &    -32768 &         - &    6.70 &     3.456 \\
   J22464980+4420030 &  53569.10 &   828 &    -32768 &         - &    6.82 &     3.473 \\
   J22464980+4420030 &  53606.14 &   283 &    -32768 &         - &    7.16 &     4.101 \\
   J22464980+4420030 &  53953.07 &   422 &    -32768 &         - &    7.15 &         - \\
   J22464980+4420030 &  53958.06 &   370 &    -32768 &         - &    7.64 &     3.922 \\
   J22464980+4420030 &  53959.07 &   392 &    -32768 &         - &    7.11 &     3.602 \\
   J22464980+4420030 &  53960.07 &   349 &    -32768 &         - &    6.63 &     3.536 \\
   J22464980+4420030 &  53955.06 &   427 &    -32768 &         - &    6.79 &     3.095 \\
   J22464980+4420030 &  53957.05 &   377 &    -32768 &         - &    7.04 &     3.699 \\
   J22515348+3145153 &  56519.98 &   255 &    -32768 &         - &   10.36 &         - \\
   J22515348+3145153 &  56520.98 &   225 &    -32768 &         - &   10.42 &     7.635 \\
   J22515348+3145153 &  56521.94 &   284 &    -32768 &         - &   10.23 &     5.738 \\
   J22515348+3145153 &  56522.94 &   261 &    -32768 &         - &   10.39 &     6.598 \\
   J23081954-1524354 &  55024.95 &   128 &      1080 &     -0.05 &   41.13 &     1.495 \\
   J23081954-1524354 &  55023.12 &    51 &    -32768 &         - &   41.55 &     0.190 \\
   J23081954-1524354 &  55024.05 &   140 &      1100 &     -0.08 &   42.58 &     0.665 \\
   J23081954-1524354 &  55025.03 &   142 &      1094 &     -0.08 &   42.28 &     2.033 \\
   J23081954-1524354 &  55025.14 &   159 &      1039 &     -0.10 &   40.19 &     0.925 \\
   J23081954-1524354 &  55023.02 &   164 &      1058 &     -0.09 &   41.71 &     1.306 \\
   J23081954-1524354 &  55023.03 &    92 &      1137 &     -0.05 &   41.45 &     2.049 \\
   J23081954-1524354 &  55023.05 &    45 &      1428 &      0.00 &   41.27 &     6.583 \\
   J23081954-1524354 &  55023.06 &   105 &      1078 &     -0.08 &   41.31 &     1.819 \\
   J23081954-1524354 &  55023.08 &   100 &      1125 &     -0.12 &   41.49 &     1.609 \\
   J23081954-1524354 &  55023.09 &    81 &      1203 &     -0.03 &   41.37 &     0.674 \\
   J23081954-1524354 &  55023.11 &    79 &    -32768 &         - &   42.13 &     0.609 \\
   J23081954-1524354 &  55024.03 &   132 &      1120 &     -0.05 &   41.98 &     1.252 \\
   J23081954-1524354 &  55024.06 &   144 &      1089 &     -0.07 &   42.43 &     5.619 \\
   J23081954-1524354 &  55024.09 &   139 &      1093 &     -0.08 &   41.30 &     2.044 \\
   J23081954-1524354 &  55024.10 &   147 &      1076 &     -0.08 &   40.47 &     1.909 \\
   J23081954-1524354 &  55024.11 &   145 &      1057 &     -0.07 &   40.89 &     0.607 \\
   J23081954-1524354 &  55024.12 &   137 &      1083 &     -0.05 &   41.21 &     0.816 \\
   J23081954-1524354 &  55024.13 &   142 &      1055 &     -0.11 &   41.58 &     0.881 \\
   J23081954-1524354 &  55024.96 &   134 &      1117 &     -0.07 &   40.61 &     6.885 \\
   J23081954-1524354 &  55024.98 &   135 &      1092 &     -0.06 &   40.76 &         - \\
   J23081954-1524354 &  55024.99 &   138 &      1048 &     -0.10 &   41.13 &     1.461 \\
   J23081954-1524354 &  55025.00 &   136 &      1082 &     -0.03 &   41.47 &    54.101 \\
   J23081954-1524354 &  55025.01 &   136 &      1084 &     -0.05 &   41.90 &         - \\
   J23081954-1524354 &  55025.05 &   133 &      1105 &     -0.04 &   41.83 &         - \\
   J23081954-1524354 &  55025.05 &   129 &      1047 &     -0.05 &   41.79 &         - \\
   J23081954-1524354 &  55025.07 &   120 &      1087 &     -0.06 &   41.47 &         - \\
   J23081954-1524354 &  55025.08 &   109 &      1124 &     -0.05 &   41.13 &         - \\
   J23081954-1524354 &  55025.09 &   123 &      1121 &     -0.06 &   41.26 &         - \\
   J23081954-1524354 &  55025.10 &   137 &      1071 &     -0.07 &   41.16 &         - \\
   J23081954-1524354 &  55025.11 &   145 &      1080 &     -0.09 &   41.19 &         - \\
   J23081954-1524354 &  55025.12 &   162 &      1067 &     -0.08 &   41.25 &         - \\
   J23081954-1524354 &  55023.04 &    35 &      1480 &     -0.11 &   39.43 &         - \\
   J23081954-1524354 &  55024.04 &   136 &      1086 &     -0.06 &   42.51 &         - \\
   J23081954-1524354 &  55024.07 &   139 &      1091 &     -0.07 &   41.63 &         - \\
   J23081954-1524354 &  55025.02 &   138 &      1062 &     -0.08 &   42.22 &         - \\
   J23081954-1524354 &  54372.91 &   169 &      1050 &     -0.07 &   41.05 &         - \\
   J23315208+1956142 &  53955.98 &   299 &    -32768 &         - &   11.06 &         - \\
   J23315244+1956138 &  53955.99 &   191 &    -32768 &         - &   16.89 &         - \\
   J23315208+1956142 &  53952.99 &   343 &    -32768 &         - &   10.75 &         - \\
   J23315244+1956138 &  53953.01 &   198 &    -32768 &         - &   16.48 &         - \\
   J23315208+1956142 &  53954.97 &   352 &    -32768 &         - &   11.13 &         - \\
   J23315244+1956138 &  53955.00 &   200 &    -32768 &         - &   16.43 &         - \\
   J23315208+1956142 &  53953.11 &   307 &    -32768 &         - &   10.85 &         - \\
   J23315244+1956138 &  53953.09 &   198 &    -32768 &         - &   16.45 &         - \\
   J23315208+1956142 &  53959.99 &   271 &    -32768 &         - &   11.49 &         - \\
   J23315244+1956138 &  53960.01 &   157 &    -32768 &         - &   16.60 &         - \\
   J23315208+1956142 &  53958.98 &   296 &    -32768 &         - &   11.21 &         - \\
   J23315244+1956138 &  53959.00 &   157 &    -32768 &         - &   16.33 &         - \\
   J23315208+1956142 &  53957.98 &   308 &    -32768 &         - &   11.09 &         - \\
   J23315244+1956138 &  53958.00 &   182 &    -32768 &         - &   16.72 &         - \\
   J23315208+1956142 &  53956.98 &   283 &    -32768 &         - &   11.01 &         - \\
   J23315244+1956138 &  53957.00 &   182 &    -32768 &         - &   16.54 &         - \\
   J23315208+1956142 &  53956.14 &   412 &    -32768 &         - &   10.99 &         - \\
   J23315244+1956138 &  53956.11 &   225 &    -32768 &         - &   16.38 &         - \\
   J23315244+1956138 &  53955.11 &   193 &    -32768 &         - &   16.40 &         - \\
   J23315208+1956142 &  53955.13 &   343 &    -32768 &         - &   10.73 &         - \\
   J23315244+1956138 &  54372.93 &   191 &    -32768 &         - &   16.28 &         - \\
   J23315244+1956138 &  54372.95 &   218 &    -32768 &         - &   16.30 &         - \\
   J23315244+1956138 &  54372.97 &   212 &    -32768 &         - &   16.33 &         - \\
   J23315244+1956138 &  54372.99 &   229 &    -32768 &         - &   16.14 &     8.021 \\
   J23315244+1956138 &  54373.02 &   206 &    -32768 &         - &   16.31 &         - \\
   J23315244+1956138 &  53958.12 &   183 &    -32768 &         - &   16.58 &         - \\
   J23315208+1956142 &  53958.14 &   294 &    -32768 &         - &   11.16 &         - \\
   J23315208+1956142 &  53960.14 &   269 &    -32768 &         - &   11.20 &         - \\
   J23315244+1956138 &  53960.12 &   155 &    -32768 &         - &   16.84 &         - \\
   J23315208+1956142 &  53957.13 &   309 &    -32768 &         - &   11.11 &         - \\
   J23315208+1956142 &  53957.12 &   311 &    -32768 &         - &   11.05 &         - \\
   J23315244+1956138 &  53957.10 &   184 &    -32768 &         - &   16.50 &    74.913 \\
   J23315244+1956138 &  53959.15 &   150 &    -32768 &         - &    5.44 &         - \\
   J23315208+1956142 &  53959.13 &   292 &    -32768 &         - &   11.11 &     7.275 \\
   J23415498+4410407 &  53546.11 &    24 &      2072 &      0.20 &    5.83 &         - \\
   J23513366+3127229 &  56904.07 &   224 &    -32768 &         - &    9.42 &     5.558 \\

